PDRF: Progressively Deblurring Radiance Field for Fast and Robust Scene Reconstruction from Blurry Images

We present Progressively Deblurring Radiance Field (PDRF), a novel approach to efficiently reconstruct high quality radiance fields from blurry images. While current State-of-The-Art (SoTA) scene reconstruction methods achieve photo-realistic rendering results from clean source views, their performances suffer when the source views are affected by blur, which is commonly observed for images in the wild. Previous deblurring methods either do not account for 3D geometry, or are computationally intense. To addresses these issues, PDRF, a progressively deblurring scheme in radiance field modeling, accurately models blur by incorporating 3D scene context. PDRF further uses an efficient importance sampling scheme, which results in fast scene optimization. Specifically, PDRF proposes a Coarse Ray Renderer to quickly estimate voxel density and feature; a Fine Voxel Renderer is then used to achieve high quality ray tracing. We perform extensive experiments and show that PDRF is 15X faster than previous SoTA while achieving better performance on both synthetic and real scenes.

==> AAAI2023 PDRF (2)/abstract.tex <==
\begin{abstract}
We present Progressively Deblurring Radiance Field (PDRF), a novel approach to efficiently reconstruct high quality radiance fields from blurry images. While current State-of-The-Art (SoTA) scene reconstruction methods achieve photo-realistic rendering results from clean source views, their performances suffer when the source views are affected by blur, which is commonly observed for images in the wild. Previous deblurring methods either do not account for 3D geometry, or are computationally intense. To addresses these issues, PDRF, a progressively deblurring scheme in radiance field modeling, accurately models blur by incorporating 3D scene context. PDRF further uses an efficient importance sampling scheme, which results in fast scene optimization. Specifically, PDRF proposes a Coarse Ray Renderer to quickly estimate voxel density and feature; a Fine Voxel Renderer is then used to achieve high quality ray tracing. We perform extensive experiments and show that PDRF is \textbf{15X faster} than previous SoTA while achieving \textbf{better performance} on both synthetic and real scenes.

%HDRF proposes a Coarse Ray Renderer, which provides fast density and color estimation. Based on these estimations, HDRF uses a Hierarchical Kernel Proposal network and a Fine Voxel Renderer to simultaneously refine the proposed kernel and color.
\end{abstract}

==> AAAI2023 PDRF (2)/backup.tex <==

% Specifically, as blurs are usually spatially variant, the same regions observed from different views have certain 3D redundancy that can be leveraged.

% when the blurs are spatially variant and can be minimized from multiple observations.

% , e.g. when camera shakes happen occasionally but not consistently. 
% it is often the case that some observations are more degraded than others, e.g. due to intermittent camera shake or changing depth of field. 
% If there exists enough clean observations of a scene from different views, a high quality radiance field can be modeled by exploring the 3D redundancy in overlapping regions.



% Even though scene reconstruction will fail when there exist a strong enough degradation to all observations, it is often the case that sufficient observations are blur-free, which allows us to explore the redundancy in multi-view 



%  Given that there exists enough clean observations of the scene from different view angles, Deblur-NeRF can obtain a relatively blur-free radiance field  despite the presence of blur. 

% we observe a region clearly from other view angles, Deblur-NeRF allows blur-free 

% Under the assumption that blur varies from different view angles and that blur-free observations can occasionally be made, the optimized radiance field can then be reasonably blur-free. 

% To this end, Deblur-NeRF~\cite{ma2022deblur} recently proposes to incorporate a blur model into the rendering pipeline. By doing so, Deblur-NeRF can synthesize high quality novel views despite the presence of blur. While this works on various blurs, one significant downside is the compute complexity in optimizing the radiance field. Deblur-NeRF models a blurry observation by blending $P$ clean pixels around its location to simulate a blur kernel convolution. Consequently, $P$ pixels need to be ray-traced from a blur-free radiance field to model a single blurry pixel. This makes Deblur-NeRF $P$ times slower than NeRF to render the same number of observations, when NeRF is already time-consuming to render. Furthermore, the pixel-wise blur is predicted based on 2D coordinates, which does not account for 3D context from the underlying radiance field and limits the blur modeling capacity. %This leads to an inability to model blur sub-optimal blur modeling when the observed blur has a significant depth variation, which is especially true for defocus blur. 

%This is especially crucial for defocus blur, as an object can be both in-focus and close to other out-of-focus objects in 2D coordinates.


% However, the proposed $P$ pixel locations are generated based on 2D pixel coordinates, which does not account for information from the underlying radiance field, e.g. the 3D context. This is especially crucial for defocus blur, as an object can be both out-of-focus and close to other in-focus objects in 2D coordinates, due to different depth. Furthermore, Deblur-NeRF is $P$ times slower than NeRF to render a single pixel at training time and requires an even longer time for optimization; therefore, a faster method is highly desired.




% it also has several limitations. Firstly, NeRF is scene-specific and requires a long optimization time; this stems from its implicit representation formulation, which requires millions of coordinate-based queries through an MLP to perform ray tracing. Many subsequent works~\cite{fridovich2022plenoxels,SunSC22,mueller2022instant,tensorf} have sought to address this issue and shown impressive progress in accelerating the optimization process. Such an acceleration is generally achieved by introducing explicit feature representations to compliment the implicit MLP, allowing for a trade-off between space and time. 

% Secondly, images acquired in the wild often suffer from degradations such as camera motion and incorrect focus. These degradations significantly impact the quality in radiance field modeling, which is now optimized from observations that are not multi-view consistent. This limits NeRF's application in more general circumstances. To this end, Deblur-NeRF~\cite{ma2022deblur} seeks to address this problem by incorporates a blur model with NeRF. This allows observed blur to be addressed as part of the rendering process, such that the estimated radiance field can stay blur-free during optimization. While this blur model works on both motion and defocus blur, it is very expensive to compute. Specifically, Deblur-NeRF formulates the blur of a pixel as an aggregation of $P$ clean pixels around the pixel. These pixel locations then need to be ray-traced from the radiance field and aggregated. However, the proposed $P$ pixel locations are generated based on 2D pixel coordinates, which does not account for information from the underlying radiance field, e.g. the 3D context. This is especially crucial for defocus blur, as an object can be both out-of-focus and close to other in-focus objects in 2D coordinates, due to different depth. Furthermore, Deblur-NeRF is $P$ times slower than NeRF to render a single pixel at training time and requires an even longer time for optimization; therefore, a faster method is highly desired.



% Under this formulation, Deblur-NeRF is $P$ times slower than NeRF to render a single pixel at training time, as shown in Fig. 1; therefore, a faster method is highly desired. Furthermore, the proposed $P$ pixel locations are generated based on 2D pixel coordinates alone, which does not account for information from the underlying radiance field, e.g. the 3D context. This is especially crucial for defocus blur, as an object can be both out-of-focus and close to other in-focus objects in 2D coordinates due to different depth.



% Since Deblur-NeRF builds its rendering on NeRF, it is reasonable to look for NeRF-accelerating methods to speed up Deblur-NeRF. There are, however, several roadblocks. NeRF-accelerating methods often achieves faster speed by representing scene opacity with an explicit voxel grid; this allows for fast voxel pruning based on their opacity, thus achieving high resolution on scene surfaces and lower compute cost overall. While such an ``online pruning" formulation works for static ray tracing, it introduces optimization issues when the rays are dynamically generated by a learning network, as gradients are propagated from, and only affecting, small segments of the rays. Furthermore, explicitly representing opacity can lead to noisy estimation on scenes with complex details, as a fixed voxel grid has less capacity and flexibility than an implicit function representation. In the case with blurry input images, this issue is exacerbated. 







% Specifically, Deblur-NeRF works by tracing multiple rays from a radiance field to render an observed pixel. This allows Deblur-NeRF to model the blurring kernel for every pixel in \emph{the rendering process} and leave the underlying radiance field to be blur-free; however, this formulation is slow to train as rendering a pixel now requires multiple traced rays. As such, a fast radiance field reconstruction method that is also robust to blurry input images is highly desired. As Deblur-NeRF is based on NeRF, potential solutions lie in accelerating NeRF, which is a topic of intense interest and progress recently. 



% Methods like Plenoxel~\cite{fridovich2022plenoxels}, DVGO~\citep{SunSC22}, Instant-NGP~\cite{mueller2022instant}, and TensoRF~\cite{tensorf} have shown impressive results in accelerating radiance field reconstruction, and achieve so by introducing explicit representational capacity to compliment the implicit rendering neural network. In particular, the opacity is often entirely represented by an explicit voxel grid, which allows for fast voxel pruning based on their opacity, thus achieving high resolution on scene surfaces and lower compute cost overall. While such an ``online pruning" formulation works for static ray tracing, it introduces optimization issues when the rays are dynamically generated by a learning network, e.g. in Deblur-NeRF, as gradients are propagated from, and only affecting, small segments of the rays. Furthermore, representing densities explicitly can lead to noisy opacity estimation on scenes with complex details, as a fixed voxel grid is less flexible than an implicit function representation. In the case with blurry input images, this issue is exacerbated; explicit opacity grids are often high noisy or collapse completely. As such, an approach that is both fast and does not rely on online pruning is desired. 


% On the other hand, deblurring has a rich research history achieves great performances by leveraging deep neural networks and supervised training. We observe a major difference between Deblur-NeRF and past literature on deblurring: Deblur-NeRF attempts to provide kernel estimation without any pixel value input, i.e. the estimation is based on \emph{pixel coordinates}; in contrast, previous works deblur based on observed pixel values and is \emph{coordinate agnostic}. Both methods have their merits; since Deblur-NeRF is a scene specific, self-supervised method, its networks can overfit to the input data and memorize the blurring kernels; however, providing color information as a part of the input can help ease the burden of memorization and allow kernel estimation to be more robust. For example, consider input images to be only partially blurred, e.g. due to defocus blur; as such, the knowledge of pixel value can allow networks to quickly converge to trivial solutions. 

%This is crucial as finer rendering requires importance sampling on opacity, as we cannot use online pruning, and kernel estimation requires color information.

% Acceleration methods for NeRF~\cite{fridovich2022plenoxels,SunSC22,tensorf} heavily rely on an explicit, volumetric opacity representation for fast voxel pruning. This is often referred to as ``coarse-to-fine'' or ``freespace skipping'', as low density voxels can be quickly eliminated from tracing. While this strategy works for static ray tracing, it introduces optimization issues when the rays are dynamically generated by PBE, as gradients only propagate from small segments of the rays. Furthermore, an explicit opacity representation is less expressive and leads to more noise when optimized on images with complex details and degradation. The combination of CRR and FVR addresses these issues by employing an importance sampling scheme similar to NeRF~\cite{DBLP:conf/eccv/MildenhallSTBRN20}; CRR further introduces an efficient combination of voxel-wise opacity estimation and ray-wise color rendering, which is different from the traditional voxel-wise rendering scheme. Despite the more sophisticated blur modeling, PDRF is significantly faster and more performance than Deblur-NeRF in modeling a blur-free radiance field, as demonstrated in Fig. 1.



% a fast, performative renderer and a kernel proposal network. We first describe PDRF's differentiable renderers, which consist of a Coarse Ray Renderer (CRR) and a Fine Voxel Renderer (FVR). CRR is lightweight and aims to provide fast opacity \emph{and} color estimations; FVR uses importance sampling based on CRR's output and a larger network to produce high quality rendering. Both CRR and FVR leverages explicit scene representations to accelerate convergence. We then describe the Progressive Kernel Proposal (PKP) module. Specifically, we follow the formulation in Eq.~(\ref{Eq:DSK}) and Eq.~(\ref{Eq:blurrender}) to model blur by estimating the sparse blur kernel and ray deformation. PKP introduces a \emph{radiance field-aware refinement} to assist the modelling, which allows the solutions to be much more specific to the 3D scene. 


















% Specifically, we make the observation that there are three variables that influence $\tilde{C}$ in Eq.~(\ref{Eq:deblur}): the locations $x_i\in \mathcal{N}(x)$, the underlying sharp pixel $C(x_i)$, and the blur kernel $h$. Amongst them, locations $x_i$ need to first be determined. To this end, Deblur-NeRF uses an MLP to predict $x_i$ and $h(x_i)$ based on the spatial and view embeddings of $x$. We argue that the modeling of blur kernels is a very challenging task to solve without color priors as input, as is done in most deblurring literature. In HKP, we break the estimation process down to multiple steps and incorporates color information to obtain fine-grained blur kernel proposals. 

% Initial Proposal: 


% \input{figures/algo}




%As such, CRR is designed for speed while still providing reasonable estimations.
% plays a crucial role in PDRF; it provides ray opacity and features estimations for ray displacement refinement in PBE and fine color rendering in FVR; as such, it needs to balance speed and accuracy.
% To achieve faster convergence, we leverage recent progress from TensoRF~\cite{tensorf} and use a decomposed tensor as the learnable, explicit feature representation; however, we do not use an explicit \emph{opacity} representation as is done by Plenoxel~\cite{fridovich2022plenoxels}, DVGO~\cite{SunSC22}, and TensoRF~\cite{tensorf}. Explicit opacity helps accelerating \emph{static} ray tracing by providing fast per-voxel opacity access, which can be use to prune off low opacity voxels. When the rays are dynamically generated by PBE, voxel pruning leads to sub-optimal learning. More specifically, PBE needs to propose multiple rays to model the blur; at the same time, gradients only back-propagate from high opacity voxels due to voxel pruning. However, high opacity voxels are not reliably estimated due to the presence of blur. To this end, an MLP-based implicit opacity representation is also more robust at handling blur than an explicit one. To accommodate PBE, we use an efficient importance sampling scheme instead of voxel pruning, and a combination of explicit features and an MLP $\mathcal{M}^{\textrm{coar}}_\sigma$ to estimate opacity: 
% be both efficient and provide good estimations of the underlying opacity and ray features for subsequent predictions. 

==> AAAI2023 PDRF (2)/conclusion.tex <==
\vspace{-0.2em}
\section{Conclusion}
In this work, we present PDRF, a novel radiance field modeling method that addresses camera motion and defocus blur in observations. PDRF is both significantly faster and more performant than previous deblurring methods. Specifically, PDRF proposes PBE, which progressively updates the blur model by incorporating information from the underlying radiance field; as such, PBE can accurately account for the observed blur. To support PBE and accelerate radiance field optimization, PDRF proposes a rendering pipeline that consists of CRR and FVR. CRR is an efficient renderer that predicts ray color based on aggregated ray features. With its lightweight design, CRR provides ray feature estimation to PBE and density estimation to FVR. FVR uses importance sampling to determine efficient voxel samples along the ray, which are then rendered by a larger network for their color and density. Both CRR and FVR use explicit feature representation to help accelerate their convergence rate. We perform extensive experiments and show that our method leads to significantly better deblurring results, especially on defocus blur. PDRF is about 15X faster than Deblur-NeRF, which is the previous SoTA. In the future, we hope to investigate more efficient ways to increase the blur model capacity without sacrificing speed.% and introduce features to model other multi-view inconsistencies, e.g. object motion.

==> AAAI2023 PDRF (2)/experiments.tex <==
\input{figures/quantitative_v2}

\section{Experiments}

\textbf{Dataset.}
We evaluate our deblurring method on the dataset provided by \cite{ma2022deblur}, which contains five synthetic scenes and twenty real world scenes. The synthetic scenes are affected by camera motion blur and defocus blur separately and have blur-free novel view groundtruth. For real world scenes, ten of them are affected by camera motion blur and the remaining ten are affected by defocus blur. While real world scenes have blur-free references, the calibration and exposure may not be consistent with source views. As such, we report quantitative evaluations, specifically PSNR and SSIM, on synthetic scenes and provide quantitative metrics on real world scenes in supplemental material. 



\noindent\textbf{Implementation Details.}
We construct PBE as a four-layer MLP with a channel size of 64 and ReLU as the activation function. The size of view embedding $l$ and ray feature $f_\textrm{ray}$ is 32 and 15. The canonical kernel locations $x'_i$ are normalized to be at most $\pm10$ pixels from $x$. For CRR, we use a decomposed feature tensor $\mathcal{G}^{\textrm{coar}}$ that represents 17 million voxels; for FVR, $\mathcal{G}^{\textrm{fine}}$ represents 134 million voxels. The channel dimension for the decomposed $\{X,Y,Z\}$ axes are $\{64,16,16\}$. For CRR, the two-layer MLP $\mathcal{M}^{\textrm{coar}}_{\sigma}$ and three-layer MLP $\mathcal{M}^{\textrm{coar}}_{r}$ have a channel size of 64 for hidden layers. The two-layer MLP $\mathcal{M}^{\textrm{fine}}_{\sigma}$ and three-layer MLP $\mathcal{M}^{\textrm{fine}}_{c}$ in FVR have a channel size of 256 for hidden layers. Overall, the model size for a single scene is 160MB in PDRF, which is smaller than TensoRF~\cite{tensorf}'s 200MB used for forward-facing scenes. PDRF is trained with a batch size of 1024 rays, each ray has coarse samples $N_c=64$ and importance sampled for $N_f=64$ additional voxels. A gamma correction function of $\hat{C}(\textbf{r}_{x})^{\frac{1}{2.2}}$ is used to account for the camera response function, following Deblur-NeRF. Each scene is trained for 25k iterations. Deblur-TensoRF, a baseline that replaces NeRF with TensoRF in Deblur-NeRF, uses explicit density and feature volumes that represent 134 million voxels and traces 160 samples per ray without pruning. Deblur-TensoRF uses a five-layer MLP for rendering, and a channel size of 128 for hidden layers. All time measurements are reported based on one NVIDIA A5000 GPU. 

\input{figures/visualization_v2}

\noindent\textbf{Ablation Study.} We compare three versions of designs to demonstrate the effectiveness of different components:

\begin{itemize}
    % \item DeblurTensoRF: Deblur-NeRF's rendering pipeline, i.e. NeRF, is replaced with TensoRF; we use 160 samples per ray for tracing. Details in supplemental material.
    \item $\textrm{PDRF}^{\textrm{single}}$-5: We use only the first stage, i.e. Eq. (4), to model blur without ray features, kernel size $P=5$.
    \item PDRF-5: PDRF with kernel size $P=5$.
    \item PDRF-10: PDRF with kernel size $P=10$.
\end{itemize}

As shown in Table 1, $\textrm{PDRF}^{\textrm{single}}$-5 is much faster than Deblur-NeRF and on par in performance, demonstrating the effectiveness of CRR and FVR; however, PDRF-5 outperforms $\textrm{PDRF}^{\textrm{single}}$-5 by introducing a second refinement stage in PBE. PDRF-5 is not significantly slower than $\textrm{PDRF}^{\textrm{single}}$-5, as CRR can obtain ray features very quickly. Finally, PDRF-10 uses a more powerful blur model by doubling the kernel size; this leads to significant performance improvement but also slower training time. An interesting direction for further optimization is to first distinguish the blurry and non-blurry regions, e.g. as shown in Fig. 3, and focus more modeling power on blurry regions. This also has applications to object motion modeling in NeRF, as oftentimes only some objects in the scene move when all observations are modeled for deformation. We demonstrate PDRF's application to \emph{object motion modeling} in the supplementary section.


\noindent\textbf{Quantitative and Visual Evaluation.}
We quantitatively and visually compare PDRF against various radiance field modeling methods in Table. 1 and Fig. 4. NeRF~\cite{DBLP:conf/eccv/MildenhallSTBRN20}, Plenoxel~\cite{fridovich2022plenoxels}, and TensoRF~\cite{tensorf} are SoTA methods that do not explicitly account for blur degradation. Plenoxel and TensoRF are significantly faster than NeRF; however, these methods often do not outperform NeRF when the inputs are blurry. In fact, TensoRF performs significantly worse and sometimes reaches collapsed solutions, e.g. with the Pool scene, where scene density is all concentrated near the camera origins. This is due to the limited capacity in TensoRF's low-rank density representation, which has more noise given blurry observations. Furthermore, the noise leads to less efficient voxel pruning and longer optimization time. Plenoxel performs better than TensoRF, but takes more memory at 2 GB per scene compared to TensoRF's 200 MB and PDRF's 160 MB features. We note that both Plenoxel and Instant-NGP~\cite{mueller2022instant} use customized CUDA kernels for acceleration and are difficult to be analyzed or modified. In particular, Instant-NGP does not have baselines for real forward-facing scenes like LLFF~\cite{DBLP:journals/tog/MildenhallSCKRN19}. We also tested on DVGO~\cite{SunSC22}; however, DVGO yields collapsed solutions for all scenes.


We then look into radiance field modeling methods that take blur into consideration. One approach is to first apply image-based or video-based deblurring methods on source views, as is done by MPR~\cite{DBLP:conf/cvpr/ZamirA0HK0021} and KPAC~\cite{9709995}. While this approach leads to some improvements, denoted as MPR+NeRF and KPAC+NeRF in Table 1, it does not explore 3D redundancy from different source views. Deblur-NeRF~\cite{ma2022deblur} uses a pixel-coordinate-based blur model before radiance field optimization and does not rely on external training data. In comparison, it outperforms all previous methods; however, Deblur-NeRF is also the most computationally demanding method and requires twenty hours to reach convergence. We create another baseline by replacing NeRF with TensoRF in Deblur-NeRF, which we named Deblur-TensoRF. Deblur-TensoRF is significantly faster than Deblur-NeRF; however, its performance is also notably worse. We contribute this again to TensoRF's compressed density representation. We also note that Deblur-TensoRF does not use voxel pruning. To demonstrate the incompatibility of voxel pruning with dynamic ray generation, we add a $\textrm{Deblur-TensoRF}^{\textrm{pru}}$ baseline in Table 1, which prunes low density voxels during training and results in significantly worse performances than Deblur-TensoRF. Our CRR+FVR design uses a combination of explicit and implicit representation to estimate density, and is both faster and more performant than Deblur-TensoRF; specifically, PDRF-5 is 15 times faster than Deblur-NeRF and takes only 80 minutes to converge. This is even faster than Deblur-TensoRF, partially due to the more efficient sampling scheme. We observe that PDRF's PBE can effectively model blur by using feature from the underlying radiance field, especially for defocus blur. This is likely because defocus blur can be much better modeled with 3D context, e.g. scene depth. Camera motion blur is less sensitive to 3D geometry of the scene; however, improvements can still be observed.

Visually, PDRF can recover very fine details both on synthesized and real scenes despite the blurry observations from neighboring source views. As shown in Fig. 4, Deblur-NeRF fails to recover details. While Deblur-TensoRF benefits from the additional blur modeling, it suffers from more noise. This can also be observed when comparing TensoRF to Plenoxel and NeRF. For more visualizations on scene density, please refer to the supplementary material section. 



==> AAAI2023 PDRF (2)/figures/PBE_vis_object_motion.tex <==
% \vspace{-0.5em}
\begin{figure}[!htb]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}[b]{cc}
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/obj_motion/016.png}
            \caption{Object motion in src. views}
            % \label{img:objmo}
        \end{subfigure} &
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/obj_motion/016_restore.png}
            \caption{PDRF reconstruction}
            % \label{pdrf_objmo}
        \end{subfigure} \\
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/obj_motion/pos_var0.png}
            \caption{$Var(\Delta x^{*}_i)$, Ma et al.}
            % \label{img:DSKobjmo}
        \end{subfigure} &
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/obj_motion/pos_var1.png}
            \caption{$Var(\Delta x_i)$, PBE}
            % \label{img:PREobjmo}
        \end{subfigure} \\
    \end{tabular}
    \caption{Visualization of object motion in (a), the foreground flower is in motion. We visualize the variance of predicted $\Delta x_i$, where higher variance correlates with more motion. Our PBE module (d) can clearly distinguish foreground details despite their proximity with background pixels; (c) can only coarsely distinguish fore/background.}
    % \label{fig:objmo}
    % \vspace{-1em}
\end{figure}

==> AAAI2023 PDRF (2)/figures/PRE_vis.tex <==
\vspace{-0.5em}
\begin{figure}[!htb]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}[b]{cc}
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/PRE_vis/001.png}
            \caption{Defocus Blur}
            \label{img:blur}
        \end{subfigure} &
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/PRE_vis/001_crop.png}
            \caption{Deblur Blur, Magnified}
            \label{}
        \end{subfigure} \\
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/PRE_vis/trans_var0.png}
            \caption{$Var(\Delta o_{x^{*}_i})$, Ma et al.}
            \label{img:DSK}
        \end{subfigure} &
        \begin{subfigure}[b]{.48\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/PRE_vis/trans_var1.png}
            \caption{$Var(\Delta o_{x_i})$, PBE}
            \label{img:PRE}
        \end{subfigure} \\
    \end{tabular}
    \caption{Visualization of defocus blur in (a), background is out-of-focus. We visualize the variance of predicted $\Delta o_{x_i}$, where higher variance correlates with more blurry regions. Our PBE module (d) can clearly distinguish foreground details despite their proximity with background pixels; (c) can only coarsely distinguish fore/background.}
    \label{fig:pre}
    \vspace{-0.5em}
\end{figure}

==> AAAI2023 PDRF (2)/figures/algo.tex <==
\newcommand{\algrule}[1][.2pt]{\par\vskip.5\baselineskip\hrule height #1\par\vskip.5\baselineskip}

\begin{algorithm}[!htb]
\SetAlgoLined
\KwIn{pixel coordinate: $x$, canonical kernel location: $\mathcal{N}(x)$, PKP-net: $H_{\Phi}$, color-net: $M_{\Theta}$, view embedding: $l$, observed color: $\tilde{C}$, ray origin and direction: $\{o,d\}$, CRR: $R_{\textrm{coarse}}$, FVR: $R_{\textrm{fine}}$}
\KwOut{ray deformation: \{$\Delta o_{x_i}, \Delta x_i$\}, kernel weight: $w_{x_i}$, rendered color: $\hat{\tilde{C}}$}
\vspace{0.2em}
\begin{algorithmic}[1]
\algrule

\STATE $\Delta x'_i = H_{\Phi}(l,x,x'_i,\emptyset)$, where $x'_i\in \mathcal{N}(x)$ 

\STATE $x_i = x'_i + \Delta x'_i, f_{\textrm{blur}}(x_i) = M_{\Theta}(\tilde{C}(x_i))$ 

\STATE $\Delta o_{x_i}, \Delta x_i, h_{x_i} = H_{\Phi}(l,x,x_i,f_{\textrm{blur}}(x_i))$ 


% \tcc{Coarse Kernel Proposal}
\algrule

\STATE $r_{x_i} = (o+\Delta o_{x_i}) + td_{x_i+\Delta x_i}$

\STATE $\hat{C}_{\textrm{coarse}}(x_i),f_{\textrm{coarse}}(x_i) = R_{\textrm{coarse}}(r_{x_i})$

\STATE $\Delta o_{x^{*}_i}, \Delta x^{*}_i, h_{x^{*}_i} = H_{\Phi}(l,x,x_i,f_{\textrm{coarse}}(x_i))$

% \tcc{Refined Kernel Proposal}
\algrule

\STATE $r^*_{x_i} = (o+\Delta o_{x^*_i}) + td_{x_i+\Delta x^*_i}$


\STATE $\hat{C}_{\textrm{fine}}(x_i) = R_{\textrm{fine}}(r^*_{x_i})$

% \tcc{Fine Rendering}

\end{algorithmic}
\caption{Progressive Kernel Proposal}
\label{alg:PKP}
\end{algorithm}

==> AAAI2023 PDRF (2)/figures/quantitative.tex <==
% \captionsetup[subfigure]{labelformat=empty}
% \newcommand{\tp}[1]{\colorbox{LimeGreen}{#1}}
\newtcbox\tp{hbox, on line, colback=LimeGreen, enhanced, frame hidden, boxrule=0pt, 
    top=-2pt, bottom=-2pt, right=-2pt, left=-2pt, sharp corners}
    
\newtcbox\seccol{hbox, on line, colback=Goldenrod, enhanced, frame hidden, boxrule=0pt, 
    top=-2pt, bottom=-2pt, right=-2pt, left=-2pt, sharp corners}
\begin{table*}[!htb]
    % \setlength{\abovecaptionskip}{5pt}
    \setlength{\tabcolsep}{0.3pt}
    \small
    \centering
    \begin{tabular}[b]{c}
        \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|cccc}
        \toprule
        %  Method & DSC1 & DSC2 & DSC3 & Avg.& NSD1 & NSD2 & NSD3 & Avg. \\
        % Brain/
            &\multicolumn{3}{c|}{\textsl{Factory}}&\multicolumn{3}{c|}{\textsl{Cozyroom}}&\multicolumn{3}{c|}{\textsl{Pool}}&\multicolumn{3}{c|}{\textsl{Tanabata}}&\multicolumn{3}{c|}{\textsl{Trolley}}&\multicolumn{4}{c}{\textsl{Average}}\\
        \midrule
         Camera Motion & \small{PSNR} & \small{SSIM} & \small{LPIPS} & \small{PSNR} & \small{SSIM} & \small{LPIPS}& \small{PSNR} & \small{SSIM} & \small{LPIPS}& \small{PSNR} & \small{SSIM} & \small{LPIPS}& \small{PSNR} & \small{SSIM} & \small{LPIPS}& \small{PSNR} & \small{SSIM} & \small{LPIPS} & Hrs\\
        \midrule
        NeRF & 19.32 & .4563 & .5304 & 25.66 & .7941 & .2288 & 30.45 & .8354 & .1932 & 22.22 & .6807 & .3653 & 21.25 & .6370 & .3633 & 23.78 & .6807 & .3362 & 5.00 \\
        
        Plenoxel & 18.42 & .4854 & .4869 & 25.56 & .8480 & .1751 & 30.13 & .8481 & .1802 & 21.67 & .6992 & .3222 & 20.81 & .6759 & .3221 & 23.31 & .7113 & .2973 & 0.42 \\
        % DVGO & 13.52 &  &  & 15.79 &  &  & 20.61 &  & & 12.99 &  &  & 14.00 &  &  & 15.38 &  & \\
        TensoRF & 18.85 & .4981 & .5104 & 24.91 & .7975 & .1917 & 15.89 & .3783 & .7473 & 21.06 & .6762 & .3275 & 20.01 & .6584& .3200 & 20.53 & .6017 & .4194 & 0.83\\
        
        \midrule
        MPR + NeRF &21.70 &.6153 &.3094 &27.88 &.8502 &.1153 &30.64 &.8385 &.1641 &22.71 &.7199 &.2509 &22.64 &.7141 &.2344 &25.11 &.7476 &.2148& 5.00\\
        % PVD + NeRF &20.33 &.5386 &.3667 &27.74 &.8296 &.1451& 27.56 &.7626 &.2148 &23.44 &.7293 &.2542& 23.81& .7351& .2567 &24.58 &.7190 &.2475&5.00\\
        Deblur-NeRF & 25.60 & .7750 & .2687 & 32.08 & .9261 & .0477 & 31.61 & .8682 & .1246 & 27.11 & .8640 & .1228 & 27.45 & .8632 & .1363 & 28.77 & .8593 & .1400 & 20.0\\
        \midrule
        
        DeblurTensoRF & 23.20 & .6560 & .3041 & 30.18 & .8890 & .0990 & 29.83 & .7956 & .1602 & 25.13 & .7891 & .1669 & 25.10 & .7894 & .1632 & 26.69 & .7838 & .1787 & 1.50\\
        
        
        $\textrm{PDRF}^{\textrm{single}}$-5 & 25.65 & .7793 & .2944 & 31.37 & .9255 & .0568 & 31.28 & .8623 & .1589 & 27.55 & .8809 & .1425 & 27.43 & .8769 & .1476 & 28.66 & .8650 & .1600&\tp{1.15}\\
        
        
        
        % $\textrm{PDRF}^{\textrm{single}}$-5 & 25.68 &  &  & 31.68 &  &  & 31.57 &  &  & 27.37 &  &  & 27.43 &  &  & 28.74 &  & \\
        PDRF-5 & 25.60 & .7786 & .3002 & \tp{32.01} & .9310 & .0518 & \tp{31.53} & \tp{.8686} & .1534 & 27.70 & .8851 & .1362 & 27.90 & .8841 & .1441 & 28.95 & .8695 &.1571&1.33\\
        PDRF-10 & \tp{26.56} & \tp{.8102} & \tp{.2648} & 31.90 & \tp{.9321} & \tp{.0443} & 31.29 & .8657 & \tp{.1430}& \tp{28.21} & \tp{.8952} & \tp{.1128} & \tp{28.48} & \tp{.8956} & \tp{.1078} & \tp{29.29} & \tp{.8798} & \tp{.1345}&2.33\\

        \bottomrule
        \toprule
         Defocus & \small{PSNR} & \small{SSIM} & \small{LPIPS} & \small{PSNR} & \small{SSIM} & \small{LPIPS}& \small{PSNR} & \small{SSIM} & \small{LPIPS}& \small{PSNR} & \small{SSIM} & \small{LPIPS}& \small{PSNR} & \small{SSIM} & \small{LPIPS}& \small{PSNR} & \small{SSIM} & \small{LPIPS} & Hrs\\
        \midrule
        NeRF & 25.36 &.7847 &.2351 &30.03 &.8926& .0885& 27.77 &.7266& .3340 &23.80 &.7811 &.2142 &22.67 &.7103 &.2799 &25.93 &.7791 &.2303& 5.00\\
        
        Plenoxel & 25.51 & .8579 & .1843 & 30.33 & .9315 & .0683 & 27.33 & .7382 & .3052 & 23.59 & .8371 & .1741 & 22.42 & .7862 & .2145 & 25.84 & .8302 & .1893& 0.42 \\
        % DVGO & 13.54 &  &  & 15.82 &  &  & 20.54 &  & & 12.99 &  &  & 13.85 &  &  & 15.35 &  & \\
        TensoRF & 25.08 & .8415 & .2197 & 29.77 & .9154 & .0861 & 16.23 & .4112 & .7585 & 22.97 & .8193 & .1868 & 22.40 & .7819 & .2249 & 23.17 & .7539 & .2952& 0.83 \\
        
        \midrule
        KPAC + NeRF &26.40 &.8194 &.1624 &28.15 &.8592 &.0815 &26.69 &.6589 &.2631 &24.81 &.8147 &.1639 &23.42 &.7495 &.2155 &25.89 &.7803 &.1773&5.00\\
        Deblur-NeRF & 28.03 &.8628 &.1127 &31.85& .9175& .0481& 30.52 &.8246& .1901 &26.25 &.8517 &.0995 &25.18 &.8067 &.1436 &28.37 &.8527 &.1188& 20.0\\
        \midrule
        
        DeblurTensoRF & 27.01 & .8257 & .1393 & 30.39 & .8882 & .0910 & 27.41 & .6841 & .2542 & 24.36 & .7835 & .1276 & 23.91 & .7593 & .1564 & 26.62 & .7882 & .1537 & 1.50\\        
        
        $\textrm{PDRF}^{\textrm{single}}$-5 & 28.33 & .8743 & .1445 & 31.78 & .9222 & .0541 & 30.43 & \seccol{.8233} & .2318 & 26.26 & .8649 & .1194 & 25.47 & .8261 & .1652 & 28.45 & .8622 & .1430&\tp{1.15}\\        
        
        PDRF-5 & \seccol{30.34} & \seccol{.9032} & \seccol{.1378} & \seccol{32.10} & \seccol{.9269} & \seccol{.0503} & \seccol{30.48} & .8262 & \seccol{.2274} & \seccol{27.31} & .8818 & .1209 & 27.05 & .8581 &  .1501 & 29.46 & .8792 & .1373&1.33\\
        PDRF-10 & \tp{30.90} & \tp{.9138} & \tp{.1111} & \tp{32.29} & \tp{.9305} & \tp{.0437} & \tp{30.97} & \tp{.8408} & \tp{.1960} & \tp{28.18} & \tp{.9006} & \tp{.0877} & \tp{28.07} &  \tp{.8799} & \tp{.1196} & \tp{30.08} & \tp{.8931} & \tp{.1116}&2.33\\
        \bottomrule
        
        \end{tabular}\\
    \end{tabular}        
    \caption{}
    \label{tab:results}
    \vspace{-1em}
\end{table*}


==> AAAI2023 PDRF (2)/figures/quantitative_real.tex <==
% \captionsetup[subfigure]{labelformat=empty}
% \newcommand{\tp}[1]{\colorbox{LimeGreen}{#1}}

\begin{table}[!htb]
    % \setlength{\abovecaptionskip}{5pt}
    \setlength{\tabcolsep}{3pt}
    % 
    \centering
    \begin{tabular}[b]{c}
        \begin{tabular}{l|ccc}
        % \multicolumn{4}{c|}{} & \multicolumn{4}{c}\\
        \toprule
           \textsl{Camera Motion}& {PSNR} & {SSIM} & {LPIPS} \\
        \midrule
        NeRF & 22.95 & 0.6333 & 0.3742 \\
        MPR+NeRF & 23.38 & 0.6655 & 0.3140 \\
        Deblur-NeRF & 25.65 & 0.7586 & 0.1818 \\
        PDRF & 25.83 & 0.7642 & 0.2032 \\
        \midrule
        \textsl{Defocus} & {PSNR} & {SSIM} & {LPIPS} \\
        \midrule
        NeRF & 22.53 & 0.6627 & 0.2480\\
        KPAC+NeRF & 23.04 & 0.6917 & 0.1847\\
        Deblur-NeRF & 23.47 & 0.7244 & 0.1220\\ 
        PDRF & 23.84 & 0.7355 & 0.1319\\
        \bottomrule
        \end{tabular}\\
    \end{tabular}        
    \caption{Quantitative comparisons of radiance field modeling methods on twenty real scenes, ten are affected by camera motion blur and another ten are affected by defocus blur. The average statistics are reported for each blur type.}
    \label{tab:results_real}
\end{table}


==> AAAI2023 PDRF (2)/figures/quantitative_v2.tex <==
% \captionsetup[subfigure]{labelformat=empty}
% \newcommand{\tp}[1]{\colorbox{LimeGreen}{#1}}

\begin{table*}[!htb]
    % \setlength{\abovecaptionskip}{5pt}
    \setlength{\tabcolsep}{3pt}
    % \small
    \centering
    \begin{tabular}[b]{c}
        \begin{tabular}{l|cc|cc|cc|cc|cc|cc|c}
        \toprule
            &\multicolumn{2}{c|}{\textsl{Factory}}&\multicolumn{2}{c|}{\textsl{Cozyroom}}&\multicolumn{2}{c|}{\textsl{Pool}}&\multicolumn{2}{c|}{\textsl{Tanabata}}&\multicolumn{2}{c|}{\textsl{Trolley}}&\multicolumn{2}{c|}{\textsl{Average}}& Time\\
        \midrule
          Camera Motion& \small{PSNR} & \small{SSIM}  & \small{PSNR} & \small{SSIM} & \small{PSNR} & \small{SSIM} & \small{PSNR} & \small{SSIM} & \small{PSNR} & \small{SSIM} & \small{PSNR} & \small{SSIM}  & Hrs\\
        \midrule
        NeRF & 19.32 & 0.4563 & 25.66 & 0.7941  & 30.45 & 0.8354 & 22.22 & 0.6807 & 21.25 & 0.6370 & 23.78 & 0.6807 & 5.00 \\
        
        Plenoxel & 18.42 & 0.4854 & 25.56 & 0.8480 & 30.13 & 0.8481 & 21.67 & 0.6992 & 20.81 & 0.6759 & 23.31 & 0.7113 & 0.42 \\
        % DVGO & 13.52 &  &  & 15.79 &  &  & 20.61 &  & & 12.99 &  &  & 14.00 &  &  & 15.38 &  & \\
        TensoRF & 18.85 & 0.4981 & 24.91 & 0.7975 & 15.89 & 0.3783 & 21.06 & 0.6762  & 20.01 & 0.6584 & 20.53 & 0.6017 & 0.83\\
        
        \midrule
        MPR + NeRF &21.70  & 0.6153 &27.88  & 0.8502 &30.64  & 0.8385 &22.71  & 0.7199  &22.64  & 0.7141 &25.11  & 0.7476 & 5.00\\
        % PVD + NeRF &20.33  & 0.5386  & 0.3667 &27.74  & 0.8296  & 0.1451& 27.56  & 0.7626  & 0.2148 &23.44  & 0.7293  & 0.2542& 23.81& 0.7351& 0.2567 &24.58  & 0.7190  & 0.2475&5.00\\
        Deblur-NeRF & 25.60 & 0.7750 &  \tp{32.08} & 0.9261 &  \tp{31.61} & \seccol{0.8682} & 27.11 & 0.8640  & 27.45 & 0.8632 & 28.77 & 0.8593 & 20.0\\
        
        Deblur-TensoRF & 23.20 & 0.6560 & 30.18 & 0.8890 & 29.83 & 0.7956 & 25.13 & 0.7891 & 25.10 & 0.7894 & 26.69 & 0.7838 & 1.50\\
        $\textrm{Deblur-TensoRF}^{\textrm{pru}}$ & 20.02 & 0.4889 & 28.00 & 0.8570 & 29.66 & 0.7968 & 22.87 & 0.7029 & 22.99 & 0.7231 & 24.71 & 0.7137 & 1.25\\
        \midrule
        
        
        $\textrm{PDRF}^{\textrm{single}}$-5 & 25.65 & 0.7793 & 31.37 & 0.9255 & 31.28 & 0.8623 & 27.55 & 0.8809 & 27.43 & 0.8769 & 28.66 & 0.8650 & \tp{1.15}\\
        
        
        
        % $\textrm{PDRF}^{\textrm{single}}$-5 & 25.68 &  &  & 31.68 &  &  & 31.57 &  &  & 27.37 &  &  & 27.43 &  &  & 28.74 &  & \\
        PDRF-5 & \seccol{25.60} & \seccol{0.7786} & \seccol{32.01} & \seccol{0.9310} & \seccol{31.53} & \tp{0.8686}  & \seccol{27.70} & \seccol{0.8851} & \seccol{27.90} & \seccol{0.8841} & \seccol{28.95} & \seccol{0.8695} &\seccol{1.33}\\
        PDRF-10 & \tp{26.56} & \tp{0.8102} & 31.90 & \tp{0.9321} & 31.29 & 0.8657 & \tp{28.21} & \tp{0.8952} & \tp{28.48} & \tp{0.8956} & \tp{29.29} & \tp{0.8798} &2.33\\

        \bottomrule
        \toprule
         Defocus & \small{PSNR} & \small{SSIM}  & \small{PSNR} & \small{SSIM} & \small{PSNR} & \small{SSIM} & \small{PSNR} & \small{SSIM} & \small{PSNR} & \small{SSIM} & \small{PSNR} & \small{SSIM}  & Hrs\\
        \midrule
        NeRF & 25.36  & 0.7847 &30.03  & 0.8926&  27.77  & 0.7266 &23.80  & 0.7811 &22.67  & 0.7103 &25.93  & 0.7791 & 5.00\\
        
        Plenoxel & 25.51 & 0.8579 & 30.33 & 0.9315 & 27.33 & 0.7382 & 23.59 & 0.8371  & 22.42 & 0.7862 & 25.84 & 0.8302 & 0.42 \\
        % DVGO & 13.54 &  &  & 15.82 &  &  & 20.54 &  & & 12.99 &  &  & 13.85 &  &  & 15.35 &  & \\
        TensoRF & 25.08 & 0.8415 & 29.77 & 0.9154 & 16.23 & 0.4112 & 22.97 & 0.8193  & 22.40 & 0.7819  & 23.17 & 0.7539 & 0.83 \\
        
        \midrule
        KPAC + NeRF &26.40  & 0.8194 &28.15  & 0.8592 &26.69  & 0.6589 &24.81  & 0.8147  &23.42  & 0.7495 &25.89  & 0.7803 &5.00\\
        Deblur-NeRF & 28.03  & 0.8628 &31.85& 0.9175& 30.52  & 0.8246& 26.25  & 0.8517  &25.18  & 0.8067  &28.37  & 0.8527 & 20.0\\
        
        Deblur-TensoRF & 27.01 & 0.8257  & 30.39 & 0.8882 & 27.41 & 0.6841 & 24.36 & 0.7835 & 23.91 & 0.7593 & 26.62 & 0.7882  & 1.50\\    
        $\textrm{Deblur-TensoRF}^{\textrm{pru}}$ & 25.55 & 0.7932 & 28.64 & 0.8777 & 27.60 & 0.6954 & 23.66 & 0.7711 & 22.51 & 0.7195 & 25.59 & 0.7714 & 1.25\\
        \midrule    
        
        $\textrm{PDRF}^{\textrm{single}}$-5 & 28.33 & 0.8743 & 31.78 & 0.9222 & 30.43 & 0.8233& 26.26 & 0.8649  & 25.47 & 0.8261 & 28.45 & 0.8622 &\tp{1.15}\\        
        
        PDRF-5 & \seccol{30.34} & \seccol{0.9032} & \seccol{32.10} & \seccol{0.9269} & \seccol{30.48} & \seccol{0.8262} & \seccol{27.31} & \seccol{0.8818} & \seccol{27.05} & \seccol{0.8581} &  \seccol{29.46} & \seccol{0.8792} &\seccol{1.33}\\
        PDRF-10 & \tp{30.90} & \tp{0.9138} & \tp{32.29} & \tp{0.9305} & \tp{30.97} & \tp{0.8408} & \tp{28.18} & \tp{0.9006} & \tp{28.07} &  \tp{0.8799} & \tp{30.08} & \tp{0.8931} &2.33\\
        \bottomrule
        
        \end{tabular}\\
    \end{tabular}        
    \caption{Quantitative comparisons of different radiance field modeling methods on five synthetic blurry scenes. We color code \tp{best} and \seccol{second best} performances.}
    \label{tab:results}
    \vspace{-1.5em}
\end{table*}


==> AAAI2023 PDRF (2)/figures/title.tex <==
\captionsetup{type=figure}
\noindent\begin{minipage}{\textwidth} 
\begin{minipage}{0.5\textwidth}
  \centering
    \begin{minipage}{0.32\textwidth}
      \centering
        % \vspace{-1.6em}
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/source/002.png}
                \caption{\fontsize{8}{10}\selectfont Source View 1}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/002_GT_marked.png}
                \caption{\fontsize{8}{10}\selectfont Novel View}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        % \vspace{-1.6em}
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/source/030.png}
                \caption{\fontsize{8}{10}\selectfont Source View 2}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/002_NeRF_crop.png}
                \caption{\fontsize{8}{10}\selectfont NeRF, 5 hrs}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/002_Plenoxel_crop.png}
                \caption{\fontsize{8}{10}\selectfont Plenoxel, 25 mins}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/002_TensoRF_crop.png}
                \caption{\fontsize{8}{10}\selectfont TensoRF, 50 mins}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/002_DeblurNeRF_crop.png}
                \caption{\fontsize{8}{10}\selectfont DeblurNeRF, \emph{20 hrs}}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/002_Ours_crop.png}
                \caption{\fontsize{8}{10}\selectfont Ours, \underline{\emph{80 mins}}}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/002_GT_crop.png}
                \caption{\fontsize{8}{10}\selectfont Ground Truth}
        \end{subfigure}  
    \end{minipage}
\end{minipage}
\begin{minipage}{0.5\textwidth}
  \centering
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/028.png}
                \caption{\fontsize{8}{10}\selectfont Source View 1}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/032_GT_marked.png}
                \caption{\fontsize{8}{10}\selectfont Novel View}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/033.png}
                \caption{\fontsize{8}{10}\selectfont Source View 2}
        \end{subfigure}  
    \end{minipage}

    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/032_NeRF_crop.png}
                \caption{\fontsize{8}{10}\selectfont NeRF, }
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/032_Plenoxel_crop.png}
                \caption{\fontsize{8}{10}\selectfont Plenoxel, }
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/032_TensoRF_crop.png}
                \caption{\fontsize{8}{10}\selectfont TensoRF}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/032_DeblurNeRF_crop.png}
                \caption{\fontsize{8}{10}\selectfont DeblurNeRF}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/032_Ours_crop.png}
                \caption{\fontsize{8}{10}\selectfont Ours}
        \end{subfigure}  
    \end{minipage}    
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/032_GT_crop.png}
                \caption{\fontsize{8}{10}\selectfont Ground Truth}
        \end{subfigure}  
    \end{minipage}
\end{minipage} 
\caption{figures} 
\label{fig:intro} 
\end{minipage}

==> AAAI2023 PDRF (2)/figures/visualization.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}[b]{ccccccc}
        % \hline
         NeRF & Plenoxel & TensoRF & Deblur-NeRF& PDRF & Ground Truth&Novel View\\

        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/002_NeRF_crop.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/002_Plenoxel_crop.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/002_TensoRF_crop.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/002_DeblurNeRF_crop.png}
            \caption{}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/002_Ours_crop.png}
            \caption{}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/002_GT_crop.png}
            \caption{}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/002_GT_marked.png}
            \caption{}
        \end{subfigure} \\

        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus/024_nerf_crop.png}
            \caption{21.71/0.7980}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus/024_plenoxel_crop.png}
            \caption{20.80/0.7780}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus/024_tensorf_crop.png}
            \caption{19.33/0.7580}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus/024_deblur_crop.png}
            \caption{\seccol{23.91/0.8692}}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus/024_ours_crop.png}
            \caption{\tp{27.92/0.9281}}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus/024_gt_crop.png}
            \caption{PSNR/SSIM}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus/024_gt_marked.png}
            \caption{}
        \end{subfigure}\\ 



        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/motion_real/021_nerf_crop.png}
            \caption{18.06/0.5609}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/motion_real/021_plenoxel_crop.png}
            \caption{17.60/0.5970}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/motion_real/021_tensorf_crop.png}
            \caption{15.39/0.3749}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/motion_real/021_deblurnerf_crop.png}
            \caption{\seccol{21.52/0.7956}}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/motion_real/021_ours_crop.png}
            \caption{\tp{23.55/0.8361}}
        \end{subfigure} & 
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/motion_real/021_gt_crop.png}
            \caption{PSNR/SSIM}
        \end{subfigure} & 
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/motion_real/021_gt_marked.png}
            \caption{}
        \end{subfigure}\\ 


        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus_real_2/024_nerf_crop.png}
            \caption{23.06/0.6711}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus_real_2/024_plenoxel_crop.png}
            \caption{22.33/0.6269}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus_real_2/024_tensorf_crop.png}
            \caption{21.07/0.7647}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus_real_2/024_deblur_crop.png}
            \caption{\tp{25.92}/\seccol{0.8513}}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus_real_2/024_ours_crop.png}
            \caption{\seccol{24.82}/\tp{0.8800}}
        \end{subfigure} & 
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus_real_2/024_gt_crop.png}
            \caption{PSNR/SSIM}
        \end{subfigure} & 
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus_real_2/024_gt_marked.png}
            \caption{}
        \end{subfigure}\\ 

        % \hline
    \end{tabular}
    \caption{Visual comparisons of different radiance field modeling methods. The first two rows are synthetic scenes with motion and defocus blur. The last two rows are real scenes with motion and defocus blur. For real scenes, the ground truth is for reference only as the exposure is often inconsistent with source views; PSNR and SSIM similarly only provide an estimate of quality. We color code \tp{best} and \seccol{second best} performances.}
    \label{tab:visualization}
    \vspace{-1.5em}
\end{figure*}

==> AAAI2023 PDRF (2)/figures/visualization_v2.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{0.5pt}
    \centering
    \small
    \begin{tabular}[b]{ccccccccc}
        % \hline
         Novel View & Src. View & NeRF & Plenoxel & TensoRF & Db-Ten.RF &Db-NeRF& PDRF & G.T.\\
        & & 5 hrs & 25 mins & 50 mins & 90 mins & 20 hrs& 80 mins& \\
        % \begin{subfigure}[b]{0.097\linewidth}
        %     \includegraphics[width=\textwidth]{figures/imgs/motion/002_NeRF_crop.png}
        %     \caption{}
        % \end{subfigure} &
        % \begin{subfigure}[b]{0.097\linewidth}
        %     \includegraphics[width=\textwidth]{figures/imgs/motion/002_Plenoxel_crop.png}
        %     \caption{}
        % \end{subfigure} &
        % \begin{subfigure}[b]{0.097\linewidth}
        %     \includegraphics[width=\textwidth]{figures/imgs/motion/002_TensoRF_crop.png}
        %     \caption{}
        % \end{subfigure} &
        % \begin{subfigure}[b]{0.097\linewidth}
        %     \includegraphics[width=\textwidth]{figures/imgs/motion/002_DeblurNeRF_crop.png}
        %     \caption{}
        % \end{subfigure} &   
        % \begin{subfigure}[b]{0.097\linewidth}
        %     \includegraphics[width=\textwidth]{figures/imgs/motion/002_Ours_crop.png}
        %     \caption{}
        % \end{subfigure} &  
        % \begin{subfigure}[b]{0.097\linewidth}
        %     \includegraphics[width=\textwidth]{figures/imgs/motion/002_GT_crop.png}
        %     \caption{}
        % \end{subfigure} &  
        % \begin{subfigure}[b]{0.097\linewidth}
        %     \includegraphics[width=\textwidth]{figures/imgs/motion/002_GT_marked.png}
        %     \caption{}
        % \end{subfigure} \\

        \begin{subfigure}[b]{0.20\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/016_gt_marked.png}
            \caption{PSNR/SSIM}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/015_crop.png}
            \caption{Motion}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/016_nerf_crop.png}
            \caption{18.98/.538}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/016_plenoxel_crop.png}
            \caption{18.51/.530}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/016_tensorf_crop.png}
            \caption{16.11/.321}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/016_deblur_tensorf_crop.png}
            \caption{22.00/.726}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/016_deblur_crop.png}
            \caption{\seccol{23.06/.805}}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/016_ours_crop.png}
            \caption{\tp{24.66/.870}}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/016_gt_crop.png}
            \caption{}
        \end{subfigure} \\ 


        \begin{subfigure}[b]{0.20\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus/024_gt_marked.png}
            \caption{PSNR/SSIM}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus/025_crop.png}
            \caption{Defocus}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus/024_nerf_crop.png}
            \caption{21.71/.798}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus/024_plenoxel_crop.png}
            \caption{20.80/.778}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus/024_tensorf_crop.png}
            \caption{19.33/.758}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus/024_deblur_tensorf_crop.png}
            \caption{19.33/.758}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus/024_deblur_crop.png}
            \caption{\seccol{23.91/.869}}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus/024_ours_crop.png}
            \caption{\tp{27.92/.928}}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus/024_gt_crop.png}
            \caption{}
        \end{subfigure} \\ 


        \begin{subfigure}[b]{0.20\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion_real/021_gt_marked.png}
            \caption{LPIPS}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion_real/022_crop.png}
            \caption{Motion}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion_real/021_nerf_crop.png}
            \caption{0.2288}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion_real/021_plenoxel_crop.png}
            \caption{0.2248}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion_real/021_tensorf_crop.png}
            \caption{0.2722}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion_real/021_deblur_tensorf_crop.png}
            \caption{0.1231}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion_real/021_deblurnerf_crop.png}
            \caption{\seccol{0.0953}}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion_real/021_ours_crop.png}
            \caption{\tp{0.0767}}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion_real/021_gt_crop.png}
            \caption{}
        \end{subfigure} \\ 


        \begin{subfigure}[b]{0.20\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus_real_2/024_gt_marked.png}
            \caption{LPIPS}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus_real_2/023_crop.png}
            \caption{Defocus}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus_real_2/024_nerf_crop.png}
            \caption{0.1219}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus_real_2/024_plenoxel_crop.png}
            \caption{0.1582}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus_real_2/024_tensorf_crop.png}
            \caption{0.1119}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus_real_2/024_deblur_tensorf_crop.png}
            \caption{0.0730}
        \end{subfigure} &
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus_real_2/024_deblur_crop.png}
            \caption{\seccol{0.0669}}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus_real_2/024_ours_crop.png}
            \caption{\tp{0.0599}}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.097\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/defocus_real_2/024_gt_crop.png}
            \caption{}
        \end{subfigure} \\ 



        % \hline
    \end{tabular}
    \caption{Visual comparisons of different radiance field modeling methods. The first two rows are synthetic scenes with motion and defocus blur. The last two rows are real scenes with motion and defocus blur. For real scenes, the ground truth is only for reference as its exposure is inconsistent with source views. Db-Ten.RF and Db-NeRF are shorthands for Deblur-TensoRF and Deblur-NeRF. We color code \tp{best} and \seccol{second best} performances.}
    \label{tab:visualization}
    \vspace{-1.5em}
\end{figure*}

==> AAAI2023 PDRF (2)/introduction.tex <==
\section{Introduction}

Reconstructing a 3D scene from 2D images is a long-standing research problem with extensive applications in robotics, site model construction, AR/VR, e-commerce, etc. Significant progress has been observed recently with developments in differentiable rendering and implicit function representation, e.g. Neural Radiance Field, or NeRF~\cite{DBLP:conf/eccv/MildenhallSTBRN20}. In this approach, scene radiance is represented as a neural network, i.e. a Multi-Layer Perceptron (MLP), which maps 3D coordinates to their respective density and color. By incorporating the MLP into ray tracing, scene radiance is optimized with a self-supervised photometric loss to satisfy multi-view observations; therefore, only calibrated images are required. This formulation produces photo-realistic scene rendering, models scene geometry, and accounts for view dependent effects.
% The scene radiance is modeled as an implicit function that maps 3D coordinates and view directions to voxel density and color. 
% NeRF models a 3D radiance field as an implicit function, which maps 3D coordinates and view directions to color and density at those locations. 
% This implicit function is parameterized as a Multi-Layer Perceptron (MLP) and trained with a self-supervising photometric loss to satisfy multi-view observations. 
% Under such a formulation, only calibrated images are required to produce photo-realistic scene rendering from novel views. Furthermore, this MLP-based implicit function can also produce the underlying 3D scene geometry and model view dependent effects.

\begin{figure}[!htb]
    \centering
      \includegraphics[width=1\linewidth,height=0.7\linewidth]{figures/PDRF_plot.png}
    \caption{Comparisons of radiance field modeling methods from \emph{blurry} images. Our proposed PDRF significantly outperforms previous methods in speed and performance. Results are aggregated from Table 1.}
    \label{fig:speed_vs_perf}
    \vspace{-1.5em}
\end{figure}


While NeRF, along with other implicit function-based methods~\cite{DBLP:conf/cvpr/ParkFSNL19,DBLP:conf/cvpr/MeschederONNG19,DBLP:conf/cvpr/ChenZ19,DBLP:conf/nips/SitzmannZW19}, marks a significant step towards photo-realistic scene reconstruction, its application in the real world is still limited. Images acquired in the wild are often affected by factors like object motion, camera motion, incorrect focus, or low light conditions. These factors can significantly impact radiance field modeling due to information loss and multi-view \emph{in}consistency. There often still exists enough information within images in the wild to model high quality radiance field, despite the unconstrained acquisition conditions. To this end, subsequent works~\cite{Mildenhall_2022_CVPR,park2021nerfies,park2021hypernerf,DBLP:conf/cvpr/PumarolaCPM21,tretschk2021nonrigid,DBLP:conf/cvpr/Martin-BruallaR21} attempt to account for these conditions with domain knowledge and estimating robust NeRF.
% RawNeRF~\cite{Mildenhall_2022_CVPR} uses an approximated tonemapped loss and variable exposure to account for low light observations. Deblur-NeRF~\cite{ma2022deblur} incorporates a blur model into the rendering pipeline such that the underlying radiance field can be blur-free. These works have shown impressive improvements in radiance field modeling from imperfect observations.


In this work, we seek to better address camera motion and defocus blur in radiance field modeling, which is commonly observed. Prior works have two drawbacks: a lack of 3D context in modeling blur and a time-consuming optimization process. In particular, Deblur-NeRF~\cite{ma2022deblur} models a blurry observation by blending $P$ clean pixels with a blur kernel; however, the pixel-wise blur is predicted based on 2D image coordinates. As we will show, this limits Deblur-NeRF's blur modeling capacity due to the lack of scene context. Since $P$ pixels need to be ray-traced to render a single blurry pixel, Deblur-NeRF is also $P$ times slower than NeRF in rendering the same number of pixels. As shown in Fig. 1, this make Deblur-NeRF very computationally demanding.%, as NeRF is already computationally demanding to optimize.

Several previous works~\cite{fridovich2022plenoxels,mueller2022instant,SunSC22,tensorf} have shown great progress in accelerating NeRF; however, they are not directly applicable to methods that dynamically generated rays to account for view inconsistencies. Specifically, these acceleration methods rely on an explicit density volume, which allows dense ray-tracing by quickly pruning away low density voxels. This strategy relies on the assumption that static rays can lead to good density approximation, which is not true when images are blurred. Voxel pruning also leads to sub-optimal learning for dynamic ray generation because gradients only propagate on parts of the ray. %Due to its limited capacity, an explicit density volume also exhibits significant noise when optimized on images with complex details and blur.

We propose a novel Progressively Deblurring Radiance Field, or PDRF. PDRF uses a Progressive Blur Estimation (PBE) module to address the lack of 3D modeling for blur. To achieve this, PBE first generates a coarse set of rays to account for blur based on 2D coordinates. PBE then traces these rays and obtains their features from the underlying radiance field. Finally, PBE refines coarse blur estimations with a second update by incorporating 3D features into blur modeling. For rendering, PDRF uses a Coarse Ray Renderer (CRR) and a Fine Voxel Renderer (FVR). CRR provides feature and density estimation for PBE and FVR respectively. In particular, CRR achieves efficiency by rendering a ray from its aggregated feature instead of rendering individual voxels. FVR focuses on quality, and uses a larger network and denser predictions for high quality view synthesis. CRR and FVR combine the use of explicit features~\cite{tensorf} and an efficient importance sampling to enable fast convergence and proper gradient updates for PBE. As demonstrated in Fig. 1, despite the more sophisticated blur modeling, PDRF is faster \emph{and} more performant than Deblur-NeRF in modeling radiance field from blurry images. In summary, our contributions can be described in three parts:











% At the core of HDRF is a Coarse Ray Renderer (CRR), which provides fast opacity and ray feature estimations. CRR performs pixel rendering from ray-tracing voxel features instead of voxel-specific rendering. This implementation is 


% . To perform deblurring, HDRF proposes a Hierarchical Kernel Proposal (HKP) network. HKP consists of a coarse and refined stage; specifically, a coarse blur kernel is first proposed for CRR to render; based on the pixel features produced by CRR, HKP further refines its kernel proposal. The refined kernel is then rendered by a combination of CRR and Fine Voxel Renderer (FVR), which takes into consideration the ray tracing direction and renders color for every voxel. By incorporating TensoRF's decomposed volume representation but rendering without online pruning, CRR and HKP is both compatible to ray optimization and extremely fast. 

\begin{enumerate}

\item We propose a Progressive Blur Estimation module, which first proposes a coarse blur model and updates it with corresponding 3D features to capture details. 

\item We propose an efficient rendering scheme, which includes a Coarse Ray Renderer and a Fine Voxel Renderer; this scheme is significantly faster than NeRF while supporting ray optimization in PBE.

\item We evaluate the overall PDRF method on synthetic and real images with blur, and find significant performance improvements compared to SoTA methods. 
\end{enumerate}


%HDRF consists of two components: a Hierarchical Kernel Proposal (HKP) network, and a fast, Coarse-to-Fine Tensorial Radiance Field (C2F-TensoRF). At the core of C2F-TensoRF lies the Coarse Ray-Renderer (CRR), which addresses multiple challenges. Specifically, CRR is very fast at estimating both color and density, which are necessary for HKP and the Fine Voxel Renderer to work. 




% we find that the DSK proposal network in Deblur-NeRF often leads to sub-optimal kernel proposal. Specifically, we observe that the kernel proposals happen before the pixel are rendered, which means that DSK has no information about the pixel values it tries to deblur other than its location. This is in contrast to many previous Deep-Learning based work which 




























==> AAAI2023 PDRF (2)/method.tex <==
\section{Progressively Deblurring Radiance Field}

\begin{figure*}[!htb]
    \centering
      \includegraphics[width=1.0\textwidth]{figures/PDRF_graph_draft_v5.png}
    \caption{PDRF is split into two stages. In the coarse stage, PBE models the blur from 2D coordinates to obtain the initial kernel locations $x^{*}_i$. We then obtain the respective ray features $f_{\textrm{ray}}(\textbf{r}_{x^{*}_i})$ from CRR. PBE then generates a second, refined blur estimate based on $\{x^{*}_i,f_{\textrm{ray}}(\textbf{r}_{x^{*}_i})\}$, and uses CRR and FVR to render the observed blurry pixel. After optimization, we can directly render from a blur-free radiance field to obtain deblurred images. }
    \label{fig:network}
    \vspace{-0.5em}
\end{figure*}

As shown in Fig.~\ref{fig:network}, PDRF consists of two parts: a Progressive Blur Estimation (PBE) module, and a rendering module that contains a Coarse Ray Renderer (CRR) and a Fine Voxel Renderer (FVR). We first describe PBE, which models blur in two stages. The coarse stage is fast and estimates blur based on 2D pixel coordinates; the finer stage updates previous results by adding ray features, such that PBE can take into account 3D scene context and model blur with more precision. We then describe CRR and FVR, which combine an efficient importance sampling scheme with explicit representations to accelerate optimization. CRR aims to provide fast ray feature and density estimations for PBE and FVR.
%; it achieves so by rendering color from aggregated ray features instead of on individual voxel. 
FVR performs importance sampling based on CRR's density estimation and have finer ray tracing resolution; it also uses a larger, voxel-wise rendering network to produce high quality view synthesis. %By combining these designs, PDRF achieves better performance in deblurring and faster speed. 

%The solution space that determines $\textbf{r}_{x_i}$, i.e. $\{o_{x_i}, d_{x_i}\}\in \mathbb{R}^{N\times P \times 6}$ for all $N$ observed pixels, is large. 

\subsection{Progressive Blur Estimation}
% \noindent\textbf{Progressive Blur Estimation.}
We follow prior works by introducing an implicit function $H$ to model blur. Specifically, $H$ estimates a number of $\textbf{r}_{x_i}$ and their blur kernel weights $h(x_i)$ for every $x$; we then follows Eq. (\ref{Eq:sparseblur}) to render the blurry observations.
%To model radiance field from blurry images, an implicit function is used to estimates $P$ number of $\textbf{r}_{x_i}$ and their blur kernel weights $h(x_i)$, which are rendered and combined following Eq. (\ref{Eq:sparseblur}). 
Since tracing $C(\textbf{r}_{x_i})$ is costly, the kernel size $P$ should be minimal. To effectively find the optimal $P$ rays to describe blur, we propose a two-stage estimation scheme. As shown in Fig. 2, the coarse blur estimation stage makes use of a canonical blur kernel location $x'_i\in \mathbb{R}^{V\times P\times 2}$ and view embedding $l\in \mathbb{R}^{V\times K}$, where $V$ is the number of source views and $K$ is the embedding size. Both $x'_i$ and $l$ are learnable parameters that effectively serve as the blur kernel and view index to $H$. We predict $\textbf{r}_{x_i}$ from $H$ in the following way:


% We further note the inputs to the blur model $G$ in Eq. (5) are 2D coordinates and their view encoding. As $G$ is a low dimensional approximation of the solution space, it naturally produces similar solutions $\{\Delta o, \Delta x'\}$ given similar $\{x,l\}$. We argue that this formulation, while efficient, limits the modeling capacity of $G$ when the blur level changes rapidly with similar $\{x,l\}$; as such, an efficient 3D representation at and around $x$ is crucial in estimating accurate $\textbf{r}_{x_i}$ and to model blur. To further motivate, we consider a complex scene in Fig.~\ref{img:blur} where the background is out-of-focus. To model blur, a key piece of information is the target pixel's depth, as pixels will have more blur when the content is further away from the focus plane. As shown in Fig.~\ref{img:DSK}, while Eq. (5) can model coarse blurry regions with a gradual change, it cannot distinguish the clean foreground details when those details are located amongst background pixels.%due to similar $\{x,l\}$. 




% which naturally constrains similar $\{x,l\}$ combinations to produce similar predictions. As we later demonstrate, this limits the modeling capacity of $G$ when blur level changes rapidly with similar $\{x,l\}$.


% As described in Eq. (5) and Eq. (6), we seek to model the blurry observation by tracing a number of $\textbf{r}_{x_i}$ from a blur-free radiance field and blending the rendered pixels. As ray-tracing is computationally expensive, the estimation of $\textbf{r}_{x_i}$ should be both precise and minimal; however, this is a challenging task. The potential solution space $\{\Delta o, \Delta x'\}\in \mathbb{R}^{N\times P \times 6}$, where $N$ is the total number of observed pixels in a scene, is very large. 

% Deblur-NeRF~\cite{ma2022deblur} predicts $\textbf{r}_{x_i}$ with an MLP network, which takes in the 2D coordinates of the observed pixel $x$ and a set of initial offsets $x'_i$ from $x$. 

% While this formulation efficiently encodes 2D pixel location, the input does not contains any 3D context. We argue that an efficient 3D representation at and around $x$ is crucial in estimating accurate $\textbf{r}_{x_i}$ and modeling blur. To motivate, consider a complex scene in Fig.~\ref{img:blur} where the background is out-of-focus. To model blur, a key piece of information is the target pixel's depth, as pixels will have more blur as their content is further away from the camera. As shown in Fig.~\ref{img:DSK}, while Deblur-NeRF can model a coarse blurry regions, it cannot distinguish the clean foreground details when those details are located amongst background pixels, limiting by their similar 2D coordinate inputs. 
 
% estimate rays $\textbf{r}_{x_i}$ and their respective contribution to the observed pixel $\tilde{C}(x)$. We note that $\textbf{r}_{x_i}$ needs to be both precise and minimal, as ray tracing is expensive. %The two parameters that determine $\textbf{r}_{x_i}$ are $\Delta o_{x_i}, \Delta x'_i$, which determine the ray origins and its direction.
% As all $\textbf{r}_{x_i}$ need to be ray-traced, we would like to estimate $\textbf{r}_{x_i}$ as precisely as possible, particularly as 
 %As such, $\textbf{r}_{x_i}$ needs to be both minimum and precise. 
%  This task is very challenging, specifically the solution space $\{\Delta o, \Delta x'\}\in \mathbb{R}^{N\times P \times 6}$, where $N$ is the total number of observed pixels in a scene and $P=|\{x_i\}|$ is the kernel size, is very large.
% Predicting $\{\Delta o, \Delta x'\}$ is also by nature a 3D task; intuitively, information about the underlying radiance field where ray-tracing happens is essential in determining $\textbf{r}_{x_i}$. The 3D context is hard to account for in the original formulation in Eq. (6), as the inputs are 2D coordinates. To this end, we introduce a ray feature modification
 
 
 
%  To address this issue, we propose a Progressive Blur Estimation (PBE) module, parameterized by an MLP network $H$. PBE has two steps; the first step makes a small modification on Eq. (5):
 
%  Intuitively, information about the underlying scene of which the rays traverse should be essential in determining $\{\Delta o, \Delta x'\}$; however, the exact method to extract such an information is unclear. Specifically, there are two questions: 1. what rays should the features be gathered, and 2. how to efficiently gather such features. 
 
 
 
 
%  As visualized in Fig. XXX, DSK~\cite{ma2022deblur} can only model the deformations very coarsely based on the coordinate information of $x$.


% We hypothesize that $\textbf{r}_{x_i}$ can be better predicted if the estimating MLP has more knowledge about the ray, particularly its ray-traced features in the radiance field. To this end, we propose a Progressive Ray Deformation (PRD) module, denoted as $H_\Phi$. PRD has two steps; the first step makes a small modification on Eq. (7):

%where $d_{x^{*}_i}$ can be computed by transforming $x^*_i$ to 3D and calculating its direction with respect to $o_{x^{*}_i}$. 

\begin{equation}
\label{Eq:PKP_1}
\begin{gathered}
    \Delta o_{x'_i}, \Delta x'_i, h'(x^*_i) = H(l,x,x'_i,\emptyset), \\
    x^{*}_i = x'_i + \Delta x'_i, o_{x^{*}_i} = o+\Delta o_{x'_i},\\
    \textbf{r}_{x^{*}_i} = o_{x^{*}_i} + td_{x^{*}_i},
\end{gathered}
\end{equation}
where $\emptyset$ is a zero vector placeholder for additional features. This initial blur model $\{\textbf{r}_{x^{*}_i}, h'(x^*_i)\}$ is similar in formulation to Deblur-NeRF~\cite{ma2022deblur} and has been shown to work reasonably well. The implicit function $H$ compactly represents all blur in the scene, and $l,x,x'_i$ are the related indices to query the specific blur model.
% In concept, $H$ is similar to the radiance field function $F$, where $l,x,x'_i$ are the related indices to be queried. As $\textbf{r}_{x^{*}_i}$ are traced and blended, $H$ then fit to the specific scenes to account for blur. 
As recent works~\cite{fridovich2022plenoxels,SunSC22,mueller2022instant,tensorf} suggest that an implicit function can be enhanced by explicit features for better and faster convergence, we hypothesize that $H$ can also benefit from additional features. 

To motivate the correct features that can help $H$ account for blur, consider a complex scene in Fig.~\ref{img:blur} where the background is out-of-focus. A key piece of information that describes blur in a pixel is its depth, as pixels have more blur when their content is further away from the camera. While $\{\textbf{r}_{x^{*}_i}, h'(x^*_i)\}$ can model a coarse blurry regions, it cannot distinguish the sharp foreground details when those details are amongst background pixels, limited by their similar 2D coordinate inputs. 
Based on this observation, we introduce a second, refinement stage that incorporates ray features $f_{\textrm{ray}}$ to $H$ for fine-grained blur modeling. As shown in Fig. 2, $f_{\textrm{ray}}(\textbf{r}_{x^{*}_i})$ is obtained by tracing and aggregating per-voxel features from the underlying radiance field. PBE performs a second inference to update $\{\textbf{r}_{x^{*}_i}, h'(x^*_i)\}$:
% where $H$ takes in an additional ray feature parameter; as we have no knowledge of the ray feature at first, a zero vector $\emptyset$ is used as a placeholder. In the second, radiance field-aware step, we update $\{\Delta o_{x'_i}, \Delta x'_i\}$ by introducing ray features $f_{\textrm{ray}}$ to $H$; the ray displacements are refined as follows:
\begin{equation}
\label{Eq:PKP_2}
\begin{gathered}
    \Delta o_{x^{*}_i}, \Delta x^*_i, h(x_i) = H(l,x,x^*_i,f_{\textrm{ray}}(\textbf{r}_{x^{*}_i})),\\
    x_i = x^*_i + \Delta x^*_i, o_{x_i} = o+\Delta o_{x^*_i},\\
    \textbf{r}_{x_i} = o_{x_i} + td_{x_i}.
\end{gathered}
\end{equation}
% where $t$ is the ray tracing step size and $d$ is the ray direction.

The updated $\{\textbf{r}_{x_i}, h'(x_i)\}$ is more accurate in describing blur, which we demonstrate in Fig.~\ref{img:DSK} and \ref{img:PRE} by measuring the variances of $\Delta o_{x^{*}_i}$ and $\Delta o_{x_i}$. When observations are already sharp, i.e. a single ray can approximate the observation, $\{\Delta o, \Delta x'\}$ should converge to similar spatial locations; when observations are blurry, $\{\Delta o, \Delta x'\}$ should be dissimilar to account for blur. Clearly, $\{\textbf{r}_{x_i}, h'(x_i)\}$ can better distinguish the clear foreground details from the blurry background.%; furthermore, edges in the blurry background also have more variance. 
While we can alternatively use a single stage to estimate $\{\Delta o, \Delta x'\}$ by replacing $\emptyset$ with $f_{\textrm{ray}}(\textbf{r}_{x^{'}_i})$ in Eq. (4), a two-stage design is still efficient since Eq. (4) computes quickly. The two-stage design also benefits from a more accurate $x^{*}_i$, which allows a more informative $f_{\textrm{ray}}(\textbf{r}_{x^{*}_i})$ .


% Both $\textbf{r}_{x_i}$ and $\textbf{r}_{x^{*}_i}$ are rendered; however, $\textbf{r}_{x^{*}_i}$ is only rendered by the coarse renderer CRR, which returns $f_{\textrm{ray}}(\textbf{r}_{x^{*}_i})$.
% While we can alternatively use a single stage to estimate $\{\Delta o, \Delta x'\}$ by replacing $\emptyset$ with $f_{\textrm{ray}}(\textbf{r}_{x^{'}_i})$ in Eq. (7), a two-stage design is similarly efficient as Eq. (7) does not require ray tracing and computes quickly. The two-stage design also benefits from a more accurate $x^{*}_i$, which allows the traced $f_{\textrm{ray}}(\textbf{r}_{x^{*}_i})$ to be more informative. We demonstrate the improvements in Fig.~\ref{img:PRE} and \ref{img:DSK} by measuring the variance of $\Delta o_{x_i}$. When observations are already sharp, $\{\Delta o, \Delta x'\}$ should converge to similar spatial locations with respect to the blur-free radiance field; when pixel observations are blurry, $\{\Delta o, \Delta x'\}$ should be dissimilar and blend a variety of rays to account for blur. PBE models blur much more accurately as it can better distinguish fore/background details.
 
 
% In addition to $\textbf{r}_{x_i}$, we always trace the original ray $\textbf{r}_{x}$. 
% In summary, PRD first finds a coarse ray deformation, then traces the deformed ray and obtains the respective ray features. Secondly, PRD finds a refined ray deformation by applying the ray feature for another inference through $H_\Phi$, which allows $H_\Phi$ to make adjustments based on the ray-traced values. We find that the refined ray deformations have a much finer spatial variation, in particular 3D spatial variation, as demonstrated in Fig. XXX. 

% In the next section, we elaborate on CRR, which enables PBE to obtain ray features and perform refined estimation. without significant computational costs. 

\input{figures/PRE_vis}
\subsection{Coarse Ray Renderer}
% \noindent\textbf{Coarse Ray Renderer}
The Coarse Ray Renderer serves two roles in PDRF: it provides coarse density estimation to FVR and ray features to PBE. CRR accomplishes this by performing a fast ray tracing.
To estimate voxel density, CRR uses a two-layer MLP $\mathcal{M}^{\textrm{coar}}_\sigma$ and an explicit feature volume $\mathcal{G}^{\textrm{coar}}$: 
\begin{equation}
\label{Eq:CRR}
    \sigma^{\textrm{coar}}_i, f^{\textrm{coar}}_{X_i} = \mathcal{M}^{\textrm{coar}}_\sigma(\gamma_{L_X}(X_i), \mathcal{G}^{\textrm{coar}}(X_i)),
\end{equation}
where $X_i$ is the traced 3D coordinates. We implement $\mathcal{G}^{\textrm{coar}}$ with tensor decomposition~\cite{tensorf} and use it to accelerate convergence for $\mathcal{M}^{\textrm{coar}}_\sigma$. 
%This design is different from previous acceleration works~\cite{fridovich2022plenoxels,SunSC22,tensorf}, which use explicit density volumes for faster access. 
We find that a purely explicit density representation used by previous methods~\cite{fridovich2022plenoxels,SunSC22,tensorf} is prone to significant noise when the observations have complex details or blur, likely due to its inflexible volumetric data structure. Therefore, Eq.~(\ref{Eq:CRR}) uses a combination of an implicit function and explicit features to ensure good density estimation. CRR further obtains an efficient ray feature representation by modifying on Eq.~(\ref{render}):
% and $\mathcal{G}^{\textrm{coar}}_f(X_i)$ is its feature as defined in Eq. (3). We further propose an efficient ray feature representation by making a modification on Eq.~(\ref{render}):
% We note that, coarse opacity estimation is a common strategy used in radiance field modelling to leverage the natural sparsity in scenes.  Some works~\cite{barron2022mipnerf360,DBLP:conf/eccv/MildenhallSTBRN20} use a dedicated MLP to estimate coarse opacity; due to the longer query time for opacity from an implicit representation, these methods estimate few voxel points first and perform importance sampling around high opacity regions for fine rendering; others~\cite{fridovich2022plenoxels,SunSC22,tensorf} use an explicit voxel grid to store opacity values, which can be accessed in fine resolution and prune off quickly on-the-fly. As online pruning leads to optimization issues for kernel proposal, importance sampling is desired. While explicit opacity representation still has a speed advantage over implicit representation, as shown in Fig. X, the speed advantage in explicit representation comes with an disadvantage in robustness to blurring noise, manifested as noisy opacity near the camera. As such, CRR adopts a dedicated MLP for opacity estimation. To render color quickly, CRR makes a modification on the formulation in Eq.~(\ref{render}) to:
\vspace{-1em}
\begin{equation}
\label{render2}
    f_{\textrm{ray}}(\textbf{r}_x)=\sum_{i=1}^{N_c} T^{\textrm{coar}}_i(1-\textrm{exp}(-\sigma^{\textrm{coar}}_i\delta_i))f^{\textrm{coar}}_{X_i},
\end{equation}
% \vspace{-0.5em}
where $f_{\textrm{ray}}(\textbf{r}_x)$ aggregates feature along ray $\textbf{r}_x$, similar to the aggregated color $C(\textbf{r}_x)$, and $N_c$ is the number of equidistant samples. We find $f_{\textrm{ray}}(\textbf{r}_x)$ to be an effective 3D representation for PBE; in particular, $f_{\textrm{ray}}(\textbf{r}_x)$ is agnostic to ray direction as the blur model in PBE is already view specific. We use $f_{\textrm{ray}}(\textbf{r}_x)$ for color rendering by another MLP $\mathcal{M}^{\textrm{coar}}_r$:
\vspace{-0.5em}
\begin{equation}
\label{render3}
    \hat{C}^{\textrm{coar}}(\textbf{r}_x)= \mathcal{M}^{\textrm{coar}}_r(f_{\textrm{ray}}(\textbf{r}_x), \gamma_{L_d}(d)).
\end{equation}
% where $\gamma_{L_d}(d)$ provides the ray direction encoding of $\textbf{r}$. 
%We find this color rendering formulation to be effective and efficient, despite the lack of per-pixel color rendering that incorporates ray direction. 
%which are of complexity $\mathcal{O}(BN)$, where $B$ is the number of ray and $N$ is the traced voxels per ray
This ray-rendering formulation has two advantages. First, it is very fast to compute; instead of querying every voxel along the ray through an MLP,  Eq.~(\ref{render3}) is only inferenced once per ray. It also serves as a coarse approximation of per-voxel rendering. Consider ray tracing when the surface density is a Dirac delta function $\sigma=\hat{\delta}(X_{\textrm{surf}})$ at a 3D location $X_{\textrm{surf}}$; this simplifies Eq. (7) and Eq. (8) to $\hat{C}^{\textrm{coar}}(\textbf{r})= \mathcal{M}^{\textrm{coar}}_r(f^{\textrm{coar}}_{X_{\textrm{surf}}}, \gamma_{L_d}(d))$, which is equivalent to per-voxel rendering. While this is the optimal solution, multi-view observations constrain $f_{\textrm{ray}}$ to coarsely represent surface features and help CRR achieve a good balance between speed and performance. CRR is first used by PBE to gather ray features and renders color based on $\{\textbf{r}_{x^*_i}, h'(x^*_i)\}$; it is then used with FVR to render colors based on the updated $\{\textbf{r}_{x_i}, h(x_i)\}$. Following Eq. (3), the predicted blurry colors are computed as follows:
\begin{equation}
\begin{gathered}
\hat{\tilde{C}}^{{\textrm{coar}}^*}(\textbf{r}_x) = \sum_{x^*_i} \hat{C}^{\textrm{coar}}(\textbf{r}_{x^*_i})h'(x^*_i), \\\hat{\tilde{C}}^{\textrm{coar}}(\textbf{r}_x) = \sum_{x_i} \hat{C}^{\textrm{coar}}(\textbf{r}_{x_i})h(x_i).
\end{gathered}
\end{equation}
Its training loss is a combined photometric loss with all blurry observation $\tilde{C}(\textbf{r}_x)$:
\begin{equation}
\mathcal{L}^{CRR}_{photo} = \lVert \hat{\tilde{C}}^{{\textrm{coar}}^*}(\textbf{r}_x)-\tilde{C}(\textbf{r}_x)\rVert^{2}_{2} + \lVert \hat{\tilde{C}}^{\textrm{coar}}(\textbf{r}_x)-\tilde{C}(\textbf{r}_x)\rVert^{2}_{2}.
\end{equation}
%In fact, we also obtain competitive results in terms of performance and speed by using Eq. (11) and Eq. (12) with TensoRF~\cite{tensorf}; demonstrations can be found in the supplemental material section.





% While this simplified formulation loses some resolution in modelling per-voxel view dependent effects, it is not completely view independent like the coarse stage in~\cite{SunSC22}; in fact, view directional effects are still reasonably modelled, as shown in Fig. Y, demonstrating the robustness of $f_{\textrm{ray}}(\textbf{r}$.

%Secondly, it doubles as an efficient pixel features to be directly transfer to HPK. 

% \noindent\textbf{Fine Voxel Renderer}
\subsection{Fine Voxel Renderer}
% While CRR is lightweight and quickly estimate $f_{\textrm{ray}}(\textbf{r}_{x_i})$ for PBE. 
The Fine Voxel Renderer leverages the density estimation from CRR and generates high quality rendering. CRR calculates weights $w_i=T_i(1-\textrm{exp}(-\sigma^{\textrm{coar}}_i\delta_i))$ for $N_c$ equidistant points in Eq. (\ref{render2}), these weights are normalized to produce a PDF of ray density. FVR uses this PDF to sample additional $N_f$ points on high density regions for finer tracing. Importance sampling scheme is used instead of voxel pruning, as voxel pruning introduces optimization issues for PBE. Specifically, previous works~\cite{fridovich2022plenoxels,SunSC22,tensorf} use explicit density volume and quickly prune off many low density voxels. While this works for \emph{static} rays, PBE dynamically generates rays $\textbf{r}_{x_i}$ based on gradients from the photometric loss. In this case, voxel pruning also eliminates gradients on many points and forces PBE to optimize $\textbf{r}_{x_i}$ base on small segments of the ray. Furthermore, high density voxels are often not correctly estimated from blurry observations and can lead to erroneous pruning. 
% When the rays are dynamically generated by PBE, voxel pruning leads to sub-optimal learning. More specifically, PBE needs to propose multiple rays to model the blur; at the same time, gradients only back-propagate from high opacity voxels due to voxel pruning. However, high opacity voxels are not reliably estimated due to the presence of blur.


% While NeRF~\cite{Mildenhall_2022_CVPR} also has an importance samp

After importance sampling, FVR uses a large MLP, which contains density and color components $\mathcal{M}^{\textrm{fine}}_\sigma$ and $\mathcal{M}^{\textrm{fine}}_c$ respectively for high quality view synthesis. The voxel density $\sigma^{\textrm{fine}}$ is obtained as follows:
\begin{equation}
    \sigma^{\textrm{fine}}, f^{\textrm{fine}}_{X_i} = \mathcal{M}^{\textrm{fine}}_\sigma(\gamma_{L_v}(X_i), \mathcal{G}^{\textrm{coar}}(X_i)\oplus \mathcal{G}^{\textrm{fine}}(X_i)),
\end{equation}
where $\oplus$ is the concatenation operation. We use an additional fine feature volume $\mathcal{G}^{\textrm{fine}}$ with the previous $\mathcal{G}^{\textrm{coar}}$ to maximize explicit feature capacity. Then, per-voxel color is rendered and aggregated as follows:
\begin{equation}
\begin{gathered} 
\textbf{c}_i = \mathcal{M}^{\textrm{fine}}_c(f^{\textrm{fine}}_{X_i}, \gamma_{L_d}(d)),\\
    \hat{C}^{\textrm{fine}}(\textbf{r}_x)=\sum_{i=1}^{N_c+N_f} T^{\textrm{fine}}_i(1-\textrm{exp}(-\sigma^{\textrm{fine}}_i\delta_i))\textbf{c}_i.
\end{gathered}
\end{equation}
A photometric loss is used for FVR, similar to CRR:
\begin{equation}
\begin{gathered}
\hat{\tilde{C}}^{\textrm{fine}}(\textbf{r}_x) = \sum_{x_i} \hat{C}^{\textrm{fine}}(\textbf{r}_{x_i})h(x_i),\\
\mathcal{L}^{FVR}_{photo} = \lVert \hat{\tilde{C}}^{\textrm{fine}}(\textbf{r}_x)-\tilde{C}(\textbf{r}_x)\rVert^{2}_{2}.
\end{gathered}
\end{equation}
Finally, the overall loss includes a total variation constraint  $\mathcal{L}^{*}_{TV}$  on the explicit feature volumes to enforce smoothness, following previous works~\cite{fridovich2022plenoxels,SunSC22,tensorf}:
\begin{equation}
\mathcal{L}_{tot} = \mathcal{L}^{CRR}_{photo} + \mathcal{L}^{FVR}_{photo} + \lambda (\mathcal{L}^{\mathcal{G}^{\textrm{coar}}}_{TV} + \mathcal{L}^{\mathcal{G}^{\textrm{fine}}}_{TV}).
\end{equation}

% where $\mathcal{L}^{*}_{TV}$ is a total variation loss used in~\cite{tensorf} and enforces smoothness in a decomposed tensor.

% PKP builds on DSK~\cite{ma2022deblur} in two ways: the estimated kernel parameters are 1. based on color information and 2. progressively updated. We outline the exact algorithm in Alg.~\ref{alg:PKP}, which is also illustrated in Fig.~\ref{fig:network}. 

% At the core of PKP is $H_\Phi$, a recurrent MLP that takes four inputs: the current pixel coordinate $x$, the kernel locations $x_i\in \mathcal{N}(x)$, the view embedding $l$, and the color feature $f(x_i)$. PKP models ray deformation $\Delta o_{x_i}, \Delta x_i$ and blur kernels $h$ simultaneously. This has been shown by~\cite{ma2022deblur} to allow sufficient flexibility in the rendering formulation to learn a blur-free radiance field. We collectively refer to $\{\Delta o_{x_i}, \Delta x_i, h\}$ as kernel proposals. PKP updates kernel proposals in three stages: color-blind proposal, blur-color proposal, and clean-color proposal. 

% \noindent\textbf{Color-blind proposal:}
% we first obtain a coarse kernel locations $x_i$ in a color-blind fashion. Specifically: 

% \begin{equation}
%     \Delta x'_i = H_{\Phi}(l,x,x'_i,\emptyset); x_i = x'_i + \Delta x'_i,
% \end{equation}

% where $x'_i$ is the starting kernel locations mentioned in Eq.~(\ref{Eq:DSK}). This step is similar to DSK; however, the goal is find coarse estimate $x_i$, which are used to sample color values from images. We call this color-blind proposal, as a zero-vector $\emptyset$ is used as the color feature. While color information related to $x$ or $x'_i$ can be generated, we empirically find that this does not lead to better deblurring performance, likely because $x$ and $x'_i$ are not informative enough yet.



% \noindent\textbf{Blur-color proposal:} Inspired by prior deblurring work, we incorporate the observed color information into refining the kernel proposal. Specifically, this process is formulated as: 

% \begin{equation}
% \begin{gathered}
%     \Delta o_{x_i}, \Delta x_i, h_{x_i} = H_{\Phi}(l,x,x_i,f_{\textrm{blur}}(x_i)),\\ f_{\textrm{blur}} = M_{\Theta}(\{\tilde{C}(x_i)\}),
% \end{gathered}
% \end{equation}

% where $\tilde{C}(x_i)$ is the observed color at $x_i$, $M_{\Theta}$ is a small MLP that extracts the color feature $f_{\textrm{blur}}$. We note that similar to a convolution operation, $M_{\Theta}$ takes the sparse patch $\{\tilde{C}(x_i)\}$ instead of extracting features point-wise. Since $x_i$ is continuous, we use trilinear interpolation to access $\tilde{C}(x_i)$. This allows $H_{\Phi}$ to update the previous estimation $x_i$ based on new information from the observation. While $\tilde{C}(x_i)$ can be useful in some situations, e.g. to assist in modelling the spatial variation of blur in the color space, we further improve the kernel proposal with estimates of clean pixels $\hat{C}(x_i)$, which the blur kernel $h(x_i)$ directly convolve with. 

% \noindent\textbf{Color-aware proposal:}




% \subsection{Fine Voxel Renderer}


==> AAAI2023 PDRF (2)/related_work.tex <==
\section{Related Work and Backgrounds}

\noindent\textbf{Motion and Defocus Deblurring.}
Motion and defocus blur are commonly observed image degradations. Blurry observations are typically modeled as convolutions between clean images and blur kernels; therefore, single image deblurring is a heavily ill-posed problem, as many solutions can lead to the same observations. Traditionally, various priors are used to constraint the solution space~\cite{DBLP:journals/tip/ChanW98,RUDIN1992259,DBLP:conf/cvpr/KrishnanTF11,DBLP:conf/cvpr/XuZJ13,5674049,DBLP:conf/nips/Levin06}. More recently, deep learning-based methods have achieved great performances by learning a more sophisticated deblurring prior in a data driven way, e.g. as a function that directly maps blurry images to clean images.~\cite{DBLP:conf/eccv/Chakrabarti16,DBLP:conf/cvpr/KupynBMMM18,DBLP:conf/cvpr/LeeSRCL21,DBLP:conf/cvpr/NahKL17,9709995,DBLP:conf/cvpr/TaoGSWJ18,DBLP:conf/cvpr/ZamirA0HK0021,DBLP:conf/cvpr/ZhangLZMSLL20} Video-based deblurring explores temporal consistency to find better solutions, e.g. through optical flow~\cite{DBLP:conf/cvpr/KimL15a,DBLP:conf/cvpr/PanBT20,DBLP:conf/cvpr/LiXZ0ZRSL21} or recurrent structures~\cite{DBLP:journals/corr/abs-2106-16028,DBLP:conf/iccv/KimLSH17,DBLP:conf/cvpr/NahSL19,DBLP:journals/tog/SonLLCL21}. 


% conventionally, blurry pixels $\tilde{C}$ are modeled by convolution operations $\ast$:
% \vspace{-0.2em}
% \begin{equation}
% \label{Eq:blur}
%     \tilde{C}(x) = C_p(x) \ast h,
% \end{equation}

\noindent\textbf{Neural Radiance Field Modeling.} Significant progress has been made in recent years on the 3D scene reconstruction task. Due to space constraints, we refer to previous surveys~\cite{DBLP:journals/pami/HanLB21,DBLP:journals/cgf/TewariFTSLSMSSN20} for a comprehensive review. We focus on neural radiance field modeling, a SoTA approach for scene reconstruction. NeRF~\cite{DBLP:conf/eccv/MildenhallSTBRN20} is a seminal work that models scene radiance with an implicit MLP function $F$. The color $\textbf{c}_i$ and density $\sigma_i$ at location $X_i\in \mathbb{R}^3$ can be queried from $F$:
\begin{equation}
\label{nerf}
\begin{gathered}
    (\textbf{c}_i,\sigma_i)=F(\gamma_{L_X}(X_i),\gamma_{L_d}(d)),
\end{gathered}
\end{equation}
where $\textbf{c}_i$ is dependent on view direction $d$, and $\gamma_{L}$ is an $L$-frequency-band embedding function that leads to better convergence~\cite{tancik2020fourfeat}. By tracing a ray at locations $X_i=o+t_{i}d$ , where $o$ is the ray origin and $t_{i}$ indicates the travel distance, the rendered color $\hat{C}(\textbf{r}_x)$ for ray $\textbf{r}_x$ is:
\begin{equation}
\label{render}
\begin{gathered}
    \hat{C}(\textbf{r}_x)=\sum_{i=1}^{N} T_i(1-\textrm{exp}(-\sigma_i\delta_i))\textbf{c}_i,\\
    T_i = \textrm{exp}(-\sum_{j=1}^{i-1}\sigma_j\delta_j),
\end{gathered}
\end{equation}
which aggregate color $\textbf{c}_i$ based current and cumulative density $\{\sigma_i, T_i\}$, modulated by distance between samples $\delta_i$. We update $F$ by constraining $\hat{C}(\textbf{r}_x)$ to be similar to observations $C(\textbf{r}_x)$ at all pixel locations $x\in \mathbb{R}^2$.
%$\lVert \hat{C}(\textbf{r}_x)-C(\textbf{r}_x)\rVert^{2}_{2}$ 
% where $\hat{C}(\textbf{r})$ is the rendered pixel from a ray $\textbf{r}$, $\sigma_i$ is the opacity for different points along the ray; $T_i = \textrm{exp}(-\sum_{j=1}^{i-1}\sigma_j\delta_j)$ is the cumulative opacity, $\delta_i=t_{i+1}-t_i$ and $t_i$ are the distance between two traced voxels and the voxel distance along the ray. NeRF estimates $\textbf{c}_i$ and $\sigma_i$ in Eq.~(\ref{render}) by modelling the underlying radiance field with a neural network function $\mathcal{F}$:
% \begin{equation}
% \label{nerf}
% \begin{gathered}
%     (\textbf{c},\sigma)=\mathcal{F}(\gamma_{L_x}(v),\gamma_{L_d}(d)),\\
%     \gamma_{L}(v)=[\textrm{sin}\pi v, \textrm{cos}\pi v, ...,\textrm{sin}2^{L-1}\pi v, \textrm{cos}2^{L-1}\pi v],
% \end{gathered}
% \end{equation}
% where $v$ is the 3D coordinate of a voxel, $d$ is the ray direction, and $\gamma_L(v)$ is the positional embedding function that is essential for better convergence~\cite{tancik2020fourfeat}. 

NeRF can produce photo-realistic renderings on novel views; however, it relies on a powerful MLP to represent the scene. This leads to a very long optimization time as millions of voxel locations need to be queried from a network. To ameliorate this issue, NeRF applies importance sampling: it first samples few equidistant locations along a ray before proposing additional points around high density regions for finer sampling. Many follow-up works seek to further accelerate NeRF optimization, generally following a space-time trade-off by introducing explicit representations to supplement implicit neural networks.
DirectVoxGo~\cite{SunSC22} proposes to use feature and density volumes to store view-invariant information and use a shallow MLP to render view-dependent color. Plenoxel~\cite{fridovich2022plenoxels} discards MLPs and uses spherical harmonics as the function basis to model view dependent effects; the voxel density and spherical harmonic coefficients are stored as volumes. A downside to using volumetric representations is the large memory footprint. To this end, Instant-NGP~\cite{mueller2022instant} uses multi-resolution hashing instead of a volume to compactly encode explicit features. TensoRF~\cite{tensorf} proposes a tensor decomposition to approximate 3D features in lower dimensions, which is more scalable to high resolution.
%For example, it can represent feature volumes $\mathcal{G}_f$ as a series of 1D vector $\textbf{v}$, $\textbf{b}$ and 2D matrices $\textbf{M}$:
%$\mathcal{G}_\sigma$ and 
% \vspace{-1em}
% \begin{equation}
% \label{Eq:tenso}
%     % \mathcal{G}_\sigma=\sum_{r=1}^{R_\sigma}\textbf{v}^{X}_{\sigma,r}\circ \textbf{M}^{YZ}_{\sigma,r} + \textbf{v}^{Y}_{\sigma,r}\circ \textbf{M}^{XZ}_{\sigma,r} + \textbf{v}^{Z}_{\sigma,r}\circ \textbf{M}^{XY}_{\sigma,r},
% % \end{equation}
% % \begin{equation}
% \begin{gathered}
%     \mathcal{G}_f=\sum_{r=1}^{R_f}\textbf{v}^{X}_{f,r}\circ \textbf{M}^{YZ}_{f,r}\circ \textbf{b}_{3r-2} + \textbf{v}^{Y}_{f,r}\circ \textbf{M}^{XZ}_{f,r}\circ \textbf{b}_{3r-1} \\+ \textbf{v}^{Z}_{f,r}\circ \textbf{M}^{XY}_{f,r}\circ \textbf{b}_{3r},
% \end{gathered}
% \end{equation}
%where $R_f$ is a hyperparameter that determine the capacity of $\mathcal{G}_f$, and $\circ$ is the outer product operation. Density volume $\mathcal{G}_\sigma$ can be similarly represented by inserting $\textbf{b}_i=1$ in Eq.~(\ref{Eq:tenso}). To retrieve feature or density at location $X$, we can directly interpolate values in $\textbf{v}$, $\textbf{b}, \textbf{M}$ with the relevant coordinates. %Notably, this can be done in PyTorch and does not require customized CUDA kernels.
% Opacity and color can then be accessed as $\sigma, c = \mathcal{G}_\sigma(v), F_\phi(\mathcal{G}_c(v), \gamma_{L_d}(d))$, where $F_\phi$ is a shallow MLP; rendering then follows Eq.~(\ref{render}). 
%$R_\sigma$ and 
%A key strategy that these methods employ is opacity-based voxel pruning. During ray tracing, these methods sample dense voxels along a ray and prune most of the voxels away based on low opacity, as explicitly represented opacity values are fast to access. In practice, this replaces importance sampling in NeRF. A downside to this pruning strategy is that it leads to optimization issues when the traced rays, i.e. ray origins and ray directions, are also learnable parameters, as it limits the gradients from most voxels. %We also observe that the explicitly estimated opacity is often nosier on real scenes with complex details as compared to NeRF. Despite the acceleration, performances on real scenes between NeRF and these acceleration methods are close. 
Another approach to accelerate NeRF is through more efficient importance sampling. Mip-NeRF360~\cite{barron2022mipnerf360} uses a small coarse network that outputs density only and is supervised by another large network. PDRF combines a novel and efficient importance sampling scheme with explicit representations to realize greater acceleration. %In spirit, this is the closest to our proposed CRR; however, CRR estimates both opacity and color to assist blur kernel estimation and also leverages explicit feature representations for speed.

% If the observed $C(r)$ is blurred, the original rendering and photometric loss alone will lead to sub-optimal Radiance Field modelling. The sub-optimalities manifest as either blurry underlying structures or noisy opacity values near the camera plane; therefore, a deblurring formulation is needed.


\noindent\textbf{NeRF Modeling With Non-Ideal Images.}
% Motion and defocus blur are commonly observed image degradations; conventionally, blurry pixels $\tilde{C}$ are modeled by convolution operations $\ast$:
% \vspace{-0.2em}
% \begin{equation}
% \label{Eq:blur}
%     \tilde{C}(x) = C_p(x) \ast h,
% \end{equation}
% where $C_p(x)$ is the clean image patch around pixel location $x$, and $h$ is the blurring kernel. In general, there is no prior knowledge of the type of blur on the image, i.e. blind deblurring, which seeks the inverse model of $h$ such that $C$ can be recovered from $\tilde{C}$. This task is heavily ill-posed but has seen much progress by leverage large-scale, supervised deep learning methods; the inverse of $h$ is often modeled by deep Convolutional Neural Networks (CNNs)~\cite{}. While the results are impressive, supervised learning requires either expensive data collection~\cite{koreanpaperonrealisticblur} or synthetic data and is often lacking in generalization. 
NeRF works well when images are clean and well-calibrated; however, images acquired in the wild are often non-ideal. Factors, such as low light, camera motion, object motion, and incorrect focus, can degrade image quality or affect multi-view consistency. Many works introduce domain knowledge to model the non-ideal contributor to observations, such that the radiance field function only models a canonical, multi-view consistent scene. RawNeRF~\cite{Mildenhall_2022_CVPR} uses an approximated tonemapped loss and variable exposure to account for low light observations. NeRF-W~\cite{DBLP:conf/cvpr/Martin-BruallaR21} uses image-specific embedding to model inconsistent appearances and transient objects. For scenes with moving objects, many works~\cite{park2021nerfies,park2021hypernerf,DBLP:conf/cvpr/PumarolaCPM21,tretschk2021nonrigid} use an implicit function to describe scene deformation, such that the rays are first deformed, then traced by a radiance field function. Recently, Deblur-NeRF~\cite{ma2022deblur} introduces an implicit function to model per-pixel blur before radiance field modeling. Specifically, the blurry observation $\tilde{C}$ is modeled as a convolution between clean pixels and a blur kernel:
% to jointly address radiance field modelling and blurry source views. Specifically, it uses a sparse blur kernel formulation, which models blur as the following:
\vspace{-0.1em}
\begin{equation}
\label{Eq:sparseblur}
    \tilde{C}(\textbf{r}_x) = \sum_{x_i\in \mathcal{N}(x)}C(\textbf{r}_{x_i})h(x_i) \text{ s.t } \sum_{x_i\in \mathcal{N}(x)}h(x_i)=1,% C_p(x) \ast h; C_p, h \in \mathbb{R}^{K\times K,}
\end{equation}
where $x_i$ denotes the clean pixel coordinates at neighboring locations $\mathcal{N}(x)$. The implicit function accounts for blur by predicting $P=|\{x_i\}|$ rays and their blending weights $h(x_i)$, which are used by a NeRF to computes $\tilde{C}(\textbf{r}_{x_i})$. %Due to the additional modeling, this method is more costly to optimize than NeRF; as such, a faster method that is suitable for dynamically updated rays is of significant interest.




% The kernel size $P=|\{x_i\}|$ is a small number, such that blur can be modeled with a sparse number of $C(\textbf{r}_{x_i})$. The sparsity is necessary due to compute limitations, as $C(\textbf{r}_{x_i})$ requires ray tracing to obtain. Deblur-NeRF then uses a Deformable Sparse Kernel (DSK) module to find $x_i$ and $h(x_i)$:

% \begin{equation}
% \label{Eq:DSK}
% \begin{gathered}
%     \Delta o_{x_i}, \Delta x'_i, h(x_i) = G(l,x,x'_i),\\
%     o_{x_i}=o+\Delta o_{x_i}, x_i=x'_i+\Delta x_i
% \end{gathered}
% \end{equation}

% where $x'_i \in \mathcal{N}(x)$ is a global set of optimizable initial kernel locations, and $l,o$ are the view embedding and camera origin for a specific source view. DSK obtains $o_{x_i}$ and $x_i$ to determine the start and end point of $\textbf{r}_{x_i}$, such that $C(x_i) = C(\textbf{r}_{x_i})$ can be traced and rendered by a NeRF. Combining Eq.~(\ref{render}) and Eq.~(\ref{Eq:sparseblur}), Deblur-NeRF renders a blurry pixel {\small$\hat{\tilde{C}}(\textbf{r}_{x})$} as follows:





% Many works~\cite{} seek to learn the inverse of $h$ through Convolutional Neural Networks (CNNs) that directly map blurry images to clean images, and supervised training, which often requires synthetic data. While blurry images can first be deblurred by these methods before used for reconstruction, the effectiveness is constrained by domain gaps and lack of generalizability from supervised training.


% \vspace{-0.2em}
% \begin{equation}
% \label{Eq:blurrender}
% \begin{gathered}
%     \hat{\tilde{C}}(\textbf{r}_{x}) = \sum_{x_i\in \mathcal{N}(x)} \hat{C}(\textbf{r}_{x_i})h(x_i),
%     % \mathcal{L}_{\tilde{photo}} = \lVert \hat{\tilde{C}}(r)-\tilde{C}(r)\rVert^{2}_{2},
% \end{gathered}
% \end{equation}

% which can be used to compute a photometric loss with blurry observations. In essence, Deblur-NeRF builds a blur model into the rendering process, allowing the radiance field to be blur-free; therefore, we can render from the radiance field without a blur model to obtain deblurred images.

%This formulation comes several advantages: 1. it is general in addressing both motion and defocus blur; 2. it relies on scene-specific self-supervision and requires no external training data. However, the inputs to the blur model $G_\Phi$ are 2D coordinates, which limits $G_\Phi$'s capacity in modeling 3D context. 
%We note that in Eq.~(\ref{Eq:DSK}), $G_\Phi$ does not consider the related color information at $x$ and $x_i$, which should be essential in determining the blur kernel. 



% allows a self-learning approach for deblurring, where $h, x_i$ are fit to specific scenes; however, a clear difference between Deblur-NeRF and previous deblurring work is that lack of direct knowledge to color values to determine the blur kernels. Specifically, $x_i$ need to be determined by DSK before $\hat{C}(\textbf{r}_{x_i})$ can be traced; however, we hypothesize that $\hat{C}(\textbf{r}_{x_i})$ is very useful in determining $x_i$ and $h_i$. To address this paradox, our proposed HPK module first estimates a coarse version of $\hat{C}(\textbf{r}_{x_i})$ and uses its related features to refine the blur kernel proposals. 

















==> backup.tex <==

% Specifically, as blurs are usually spatially variant, the same regions observed from different views have certain 3D redundancy that can be leveraged.

% when the blurs are spatially variant and can be minimized from multiple observations.

% , e.g. when camera shakes happen occasionally but not consistently. 
% it is often the case that some observations are more degraded than others, e.g. due to intermittent camera shake or changing depth of field. 
% If there exists enough clean observations of a scene from different views, a high quality radiance field can be modeled by exploring the 3D redundancy in overlapping regions.



% Even though scene reconstruction will fail when there exist a strong enough degradation to all observations, it is often the case that sufficient observations are blur-free, which allows us to explore the redundancy in multi-view 



%  Given that there exists enough clean observations of the scene from different view angles, Deblur-NeRF can obtain a relatively blur-free radiance field  despite the presence of blur. 

% we observe a region clearly from other view angles, Deblur-NeRF allows blur-free 

% Under the assumption that blur varies from different view angles and that blur-free observations can occasionally be made, the optimized radiance field can then be reasonably blur-free. 

% To this end, Deblur-NeRF~\cite{ma2022deblur} recently proposes to incorporate a blur model into the rendering pipeline. By doing so, Deblur-NeRF can synthesize high quality novel views despite the presence of blur. While this works on various blurs, one significant downside is the compute complexity in optimizing the radiance field. Deblur-NeRF models a blurry observation by blending $P$ clean pixels around its location to simulate a blur kernel convolution. Consequently, $P$ pixels need to be ray-traced from a blur-free radiance field to model a single blurry pixel. This makes Deblur-NeRF $P$ times slower than NeRF to render the same number of observations, when NeRF is already time-consuming to render. Furthermore, the pixel-wise blur is predicted based on 2D coordinates, which does not account for 3D context from the underlying radiance field and limits the blur modeling capacity. %This leads to an inability to model blur sub-optimal blur modeling when the observed blur has a significant depth variation, which is especially true for defocus blur. 

%This is especially crucial for defocus blur, as an object can be both in-focus and close to other out-of-focus objects in 2D coordinates.


% However, the proposed $P$ pixel locations are generated based on 2D pixel coordinates, which does not account for information from the underlying radiance field, e.g. the 3D context. This is especially crucial for defocus blur, as an object can be both out-of-focus and close to other in-focus objects in 2D coordinates, due to different depth. Furthermore, Deblur-NeRF is $P$ times slower than NeRF to render a single pixel at training time and requires an even longer time for optimization; therefore, a faster method is highly desired.




% it also has several limitations. Firstly, NeRF is scene-specific and requires a long optimization time; this stems from its implicit representation formulation, which requires millions of coordinate-based queries through an MLP to perform ray tracing. Many subsequent works~\cite{fridovich2022plenoxels,SunSC22,mueller2022instant,tensorf} have sought to address this issue and shown impressive progress in accelerating the optimization process. Such an acceleration is generally achieved by introducing explicit feature representations to compliment the implicit MLP, allowing for a trade-off between space and time. 

% Secondly, images acquired in the wild often suffer from degradations such as camera motion and incorrect focus. These degradations significantly impact the quality in radiance field modeling, which is now optimized from observations that are not multi-view consistent. This limits NeRF's application in more general circumstances. To this end, Deblur-NeRF~\cite{ma2022deblur} seeks to address this problem by incorporates a blur model with NeRF. This allows observed blur to be addressed as part of the rendering process, such that the estimated radiance field can stay blur-free during optimization. While this blur model works on both motion and defocus blur, it is very expensive to compute. Specifically, Deblur-NeRF formulates the blur of a pixel as an aggregation of $P$ clean pixels around the pixel. These pixel locations then need to be ray-traced from the radiance field and aggregated. However, the proposed $P$ pixel locations are generated based on 2D pixel coordinates, which does not account for information from the underlying radiance field, e.g. the 3D context. This is especially crucial for defocus blur, as an object can be both out-of-focus and close to other in-focus objects in 2D coordinates, due to different depth. Furthermore, Deblur-NeRF is $P$ times slower than NeRF to render a single pixel at training time and requires an even longer time for optimization; therefore, a faster method is highly desired.



% Under this formulation, Deblur-NeRF is $P$ times slower than NeRF to render a single pixel at training time, as shown in Fig. 1; therefore, a faster method is highly desired. Furthermore, the proposed $P$ pixel locations are generated based on 2D pixel coordinates alone, which does not account for information from the underlying radiance field, e.g. the 3D context. This is especially crucial for defocus blur, as an object can be both out-of-focus and close to other in-focus objects in 2D coordinates due to different depth.



% Since Deblur-NeRF builds its rendering on NeRF, it is reasonable to look for NeRF-accelerating methods to speed up Deblur-NeRF. There are, however, several roadblocks. NeRF-accelerating methods often achieves faster speed by representing scene opacity with an explicit voxel grid; this allows for fast voxel pruning based on their opacity, thus achieving high resolution on scene surfaces and lower compute cost overall. While such an ``online pruning" formulation works for static ray tracing, it introduces optimization issues when the rays are dynamically generated by a learning network, as gradients are propagated from, and only affecting, small segments of the rays. Furthermore, explicitly representing opacity can lead to noisy estimation on scenes with complex details, as a fixed voxel grid has less capacity and flexibility than an implicit function representation. In the case with blurry input images, this issue is exacerbated. 







% Specifically, Deblur-NeRF works by tracing multiple rays from a radiance field to render an observed pixel. This allows Deblur-NeRF to model the blurring kernel for every pixel in \emph{the rendering process} and leave the underlying radiance field to be blur-free; however, this formulation is slow to train as rendering a pixel now requires multiple traced rays. As such, a fast radiance field reconstruction method that is also robust to blurry input images is highly desired. As Deblur-NeRF is based on NeRF, potential solutions lie in accelerating NeRF, which is a topic of intense interest and progress recently. 



% Methods like Plenoxel~\cite{fridovich2022plenoxels}, DVGO~\citep{SunSC22}, Instant-NGP~\cite{mueller2022instant}, and TensoRF~\cite{tensorf} have shown impressive results in accelerating radiance field reconstruction, and achieve so by introducing explicit representational capacity to compliment the implicit rendering neural network. In particular, the opacity is often entirely represented by an explicit voxel grid, which allows for fast voxel pruning based on their opacity, thus achieving high resolution on scene surfaces and lower compute cost overall. While such an ``online pruning" formulation works for static ray tracing, it introduces optimization issues when the rays are dynamically generated by a learning network, e.g. in Deblur-NeRF, as gradients are propagated from, and only affecting, small segments of the rays. Furthermore, representing densities explicitly can lead to noisy opacity estimation on scenes with complex details, as a fixed voxel grid is less flexible than an implicit function representation. In the case with blurry input images, this issue is exacerbated; explicit opacity grids are often high noisy or collapse completely. As such, an approach that is both fast and does not rely on online pruning is desired. 


% On the other hand, deblurring has a rich research history achieves great performances by leveraging deep neural networks and supervised training. We observe a major difference between Deblur-NeRF and past literature on deblurring: Deblur-NeRF attempts to provide kernel estimation without any pixel value input, i.e. the estimation is based on \emph{pixel coordinates}; in contrast, previous works deblur based on observed pixel values and is \emph{coordinate agnostic}. Both methods have their merits; since Deblur-NeRF is a scene specific, self-supervised method, its networks can overfit to the input data and memorize the blurring kernels; however, providing color information as a part of the input can help ease the burden of memorization and allow kernel estimation to be more robust. For example, consider input images to be only partially blurred, e.g. due to defocus blur; as such, the knowledge of pixel value can allow networks to quickly converge to trivial solutions. 

%This is crucial as finer rendering requires importance sampling on opacity, as we cannot use online pruning, and kernel estimation requires color information.

% Acceleration methods for NeRF~\cite{fridovich2022plenoxels,SunSC22,tensorf} heavily rely on an explicit, volumetric opacity representation for fast voxel pruning. This is often referred to as ``coarse-to-fine'' or ``freespace skipping'', as low density voxels can be quickly eliminated from tracing. While this strategy works for static ray tracing, it introduces optimization issues when the rays are dynamically generated by PBE, as gradients only propagate from small segments of the rays. Furthermore, an explicit opacity representation is less expressive and leads to more noise when optimized on images with complex details and degradation. The combination of CRR and FVR addresses these issues by employing an importance sampling scheme similar to NeRF~\cite{DBLP:conf/eccv/MildenhallSTBRN20}; CRR further introduces an efficient combination of voxel-wise opacity estimation and ray-wise color rendering, which is different from the traditional voxel-wise rendering scheme. Despite the more sophisticated blur modeling, PDRF is significantly faster and more performance than Deblur-NeRF in modeling a blur-free radiance field, as demonstrated in Fig. 1.



% a fast, performative renderer and a kernel proposal network. We first describe PDRF's differentiable renderers, which consist of a Coarse Ray Renderer (CRR) and a Fine Voxel Renderer (FVR). CRR is lightweight and aims to provide fast opacity \emph{and} color estimations; FVR uses importance sampling based on CRR's output and a larger network to produce high quality rendering. Both CRR and FVR leverages explicit scene representations to accelerate convergence. We then describe the Progressive Kernel Proposal (PKP) module. Specifically, we follow the formulation in Eq.~(\ref{Eq:DSK}) and Eq.~(\ref{Eq:blurrender}) to model blur by estimating the sparse blur kernel and ray deformation. PKP introduces a \emph{radiance field-aware refinement} to assist the modelling, which allows the solutions to be much more specific to the 3D scene. 


















% Specifically, we make the observation that there are three variables that influence $\tilde{C}$ in Eq.~(\ref{Eq:deblur}): the locations $x_i\in \mathcal{N}(x)$, the underlying sharp pixel $C(x_i)$, and the blur kernel $h$. Amongst them, locations $x_i$ need to first be determined. To this end, Deblur-NeRF uses an MLP to predict $x_i$ and $h(x_i)$ based on the spatial and view embeddings of $x$. We argue that the modeling of blur kernels is a very challenging task to solve without color priors as input, as is done in most deblurring literature. In HKP, we break the estimation process down to multiple steps and incorporates color information to obtain fine-grained blur kernel proposals. 

% Initial Proposal: 


% \input{figures/algo}




%As such, CRR is designed for speed while still providing reasonable estimations.
% plays a crucial role in PDRF; it provides ray opacity and features estimations for ray displacement refinement in PBE and fine color rendering in FVR; as such, it needs to balance speed and accuracy.
% To achieve faster convergence, we leverage recent progress from TensoRF~\cite{tensorf} and use a decomposed tensor as the learnable, explicit feature representation; however, we do not use an explicit \emph{opacity} representation as is done by Plenoxel~\cite{fridovich2022plenoxels}, DVGO~\cite{SunSC22}, and TensoRF~\cite{tensorf}. Explicit opacity helps accelerating \emph{static} ray tracing by providing fast per-voxel opacity access, which can be use to prune off low opacity voxels. When the rays are dynamically generated by PBE, voxel pruning leads to sub-optimal learning. More specifically, PBE needs to propose multiple rays to model the blur; at the same time, gradients only back-propagate from high opacity voxels due to voxel pruning. However, high opacity voxels are not reliably estimated due to the presence of blur. To this end, an MLP-based implicit opacity representation is also more robust at handling blur than an explicit one. To accommodate PBE, we use an efficient importance sampling scheme instead of voxel pruning, and a combination of explicit features and an MLP $\mathcal{M}^{\textrm{coar}}_\sigma$ to estimate opacity: 
% be both efficient and provide good estimations of the underlying opacity and ray features for subsequent predictions. 

==> figures/algo.tex <==
\newcommand{\algrule}[1][.2pt]{\par\vskip.5\baselineskip\hrule height #1\par\vskip.5\baselineskip}

\begin{algorithm}[!htb]
\SetAlgoLined
\KwIn{pixel coordinate: $x$, canonical kernel location: $\mathcal{N}(x)$, PKP-net: $H_{\Phi}$, color-net: $M_{\Theta}$, view embedding: $l$, observed color: $\tilde{C}$, ray origin and direction: $\{o,d\}$, CRR: $R_{\textrm{coarse}}$, FVR: $R_{\textrm{fine}}$}
\KwOut{ray deformation: \{$\Delta o_{x_i}, \Delta x_i$\}, kernel weight: $w_{x_i}$, rendered color: $\hat{\tilde{C}}$}
\vspace{0.2em}
\begin{algorithmic}[1]
\algrule

\STATE $\Delta x'_i = H_{\Phi}(l,x,x'_i,\emptyset)$, where $x'_i\in \mathcal{N}(x)$ 

\STATE $x_i = x'_i + \Delta x'_i, f_{\textrm{blur}}(x_i) = M_{\Theta}(\tilde{C}(x_i))$ 

\STATE $\Delta o_{x_i}, \Delta x_i, h_{x_i} = H_{\Phi}(l,x,x_i,f_{\textrm{blur}}(x_i))$ 


% \tcc{Coarse Kernel Proposal}
\algrule

\STATE $r_{x_i} = (o+\Delta o_{x_i}) + td_{x_i+\Delta x_i}$

\STATE $\hat{C}_{\textrm{coarse}}(x_i),f_{\textrm{coarse}}(x_i) = R_{\textrm{coarse}}(r_{x_i})$

\STATE $\Delta o_{x^{*}_i}, \Delta x^{*}_i, h_{x^{*}_i} = H_{\Phi}(l,x,x_i,f_{\textrm{coarse}}(x_i))$

% \tcc{Refined Kernel Proposal}
\algrule

\STATE $r^*_{x_i} = (o+\Delta o_{x^*_i}) + td_{x_i+\Delta x^*_i}$


\STATE $\hat{C}_{\textrm{fine}}(x_i) = R_{\textrm{fine}}(r^*_{x_i})$

% \tcc{Fine Rendering}

\end{algorithmic}
\caption{Progressive Kernel Proposal}
\label{alg:PKP}
\end{algorithm}

==> figures/quantitative.tex <==
% \captionsetup[subfigure]{labelformat=empty}
% \newcommand{\tp}[1]{\colorbox{LimeGreen}{#1}}
\newtcbox\tp{hbox, on line, colback=LimeGreen, enhanced, frame hidden, boxrule=0pt, 
    top=-2pt, bottom=-2pt, right=-2pt, left=-2pt, sharp corners}
    
\newtcbox\seccol{hbox, on line, colback=Goldenrod, enhanced, frame hidden, boxrule=0pt, 
    top=-2pt, bottom=-2pt, right=-2pt, left=-2pt, sharp corners}
\begin{table*}[!htb]
    % \setlength{\abovecaptionskip}{5pt}
    \setlength{\tabcolsep}{0.3pt}
    \small
    \centering
    \begin{tabular}[b]{c}
        \begin{tabular}{l|ccc|ccc|ccc|ccc|ccc|cccc}
        \toprule
        %  Method & DSC1 & DSC2 & DSC3 & Avg.& NSD1 & NSD2 & NSD3 & Avg. \\
        % Brain/
            &\multicolumn{3}{c|}{\textsl{Factory}}&\multicolumn{3}{c|}{\textsl{Cozyroom}}&\multicolumn{3}{c|}{\textsl{Pool}}&\multicolumn{3}{c|}{\textsl{Tanabata}}&\multicolumn{3}{c|}{\textsl{Trolley}}&\multicolumn{4}{c}{\textsl{Average}}\\
        \midrule
         Camera Motion & \small{PSNR} & \small{SSIM} & \small{LPIPS} & \small{PSNR} & \small{SSIM} & \small{LPIPS}& \small{PSNR} & \small{SSIM} & \small{LPIPS}& \small{PSNR} & \small{SSIM} & \small{LPIPS}& \small{PSNR} & \small{SSIM} & \small{LPIPS}& \small{PSNR} & \small{SSIM} & \small{LPIPS} & Hrs\\
        \midrule
        NeRF & 19.32 & .4563 & .5304 & 25.66 & .7941 & .2288 & 30.45 & .8354 & .1932 & 22.22 & .6807 & .3653 & 21.25 & .6370 & .3633 & 23.78 & .6807 & .3362 & 5.00 \\
        
        Plenoxel & 18.42 & .4854 & .4869 & 25.56 & .8480 & .1751 & 30.13 & .8481 & .1802 & 21.67 & .6992 & .3222 & 20.81 & .6759 & .3221 & 23.31 & .7113 & .2973 & 0.42 \\
        % DVGO & 13.52 &  &  & 15.79 &  &  & 20.61 &  & & 12.99 &  &  & 14.00 &  &  & 15.38 &  & \\
        TensoRF & 18.85 & .4981 & .5104 & 24.91 & .7975 & .1917 & 15.89 & .3783 & .7473 & 21.06 & .6762 & .3275 & 20.01 & .6584& .3200 & 20.53 & .6017 & .4194 & 0.83\\
        
        \midrule
        MPR + NeRF &21.70 &.6153 &.3094 &27.88 &.8502 &.1153 &30.64 &.8385 &.1641 &22.71 &.7199 &.2509 &22.64 &.7141 &.2344 &25.11 &.7476 &.2148& 5.00\\
        % PVD + NeRF &20.33 &.5386 &.3667 &27.74 &.8296 &.1451& 27.56 &.7626 &.2148 &23.44 &.7293 &.2542& 23.81& .7351& .2567 &24.58 &.7190 &.2475&5.00\\
        Deblur-NeRF & 25.60 & .7750 & .2687 & 32.08 & .9261 & .0477 & 31.61 & .8682 & .1246 & 27.11 & .8640 & .1228 & 27.45 & .8632 & .1363 & 28.77 & .8593 & .1400 & 20.0\\
        \midrule
        
        DeblurTensoRF & 23.20 & .6560 & .3041 & 30.18 & .8890 & .0990 & 29.83 & .7956 & .1602 & 25.13 & .7891 & .1669 & 25.10 & .7894 & .1632 & 26.69 & .7838 & .1787 & 1.50\\
        
        
        $\textrm{PDRF}^{\textrm{single}}$-5 & 25.65 & .7793 & .2944 & 31.37 & .9255 & .0568 & 31.28 & .8623 & .1589 & 27.55 & .8809 & .1425 & 27.43 & .8769 & .1476 & 28.66 & .8650 & .1600&\tp{1.15}\\
        
        
        
        % $\textrm{PDRF}^{\textrm{single}}$-5 & 25.68 &  &  & 31.68 &  &  & 31.57 &  &  & 27.37 &  &  & 27.43 &  &  & 28.74 &  & \\
        PDRF-5 & 25.60 & .7786 & .3002 & \tp{32.01} & .9310 & .0518 & \tp{31.53} & \tp{.8686} & .1534 & 27.70 & .8851 & .1362 & 27.90 & .8841 & .1441 & 28.95 & .8695 &.1571&1.33\\
        PDRF-10 & \tp{26.56} & \tp{.8102} & \tp{.2648} & 31.90 & \tp{.9321} & \tp{.0443} & 31.29 & .8657 & \tp{.1430}& \tp{28.21} & \tp{.8952} & \tp{.1128} & \tp{28.48} & \tp{.8956} & \tp{.1078} & \tp{29.29} & \tp{.8798} & \tp{.1345}&2.33\\

        \bottomrule
        \toprule
         Defocus & \small{PSNR} & \small{SSIM} & \small{LPIPS} & \small{PSNR} & \small{SSIM} & \small{LPIPS}& \small{PSNR} & \small{SSIM} & \small{LPIPS}& \small{PSNR} & \small{SSIM} & \small{LPIPS}& \small{PSNR} & \small{SSIM} & \small{LPIPS}& \small{PSNR} & \small{SSIM} & \small{LPIPS} & Hrs\\
        \midrule
        NeRF & 25.36 &.7847 &.2351 &30.03 &.8926& .0885& 27.77 &.7266& .3340 &23.80 &.7811 &.2142 &22.67 &.7103 &.2799 &25.93 &.7791 &.2303& 5.00\\
        
        Plenoxel & 25.51 & .8579 & .1843 & 30.33 & .9315 & .0683 & 27.33 & .7382 & .3052 & 23.59 & .8371 & .1741 & 22.42 & .7862 & .2145 & 25.84 & .8302 & .1893& 0.42 \\
        % DVGO & 13.54 &  &  & 15.82 &  &  & 20.54 &  & & 12.99 &  &  & 13.85 &  &  & 15.35 &  & \\
        TensoRF & 25.08 & .8415 & .2197 & 29.77 & .9154 & .0861 & 16.23 & .4112 & .7585 & 22.97 & .8193 & .1868 & 22.40 & .7819 & .2249 & 23.17 & .7539 & .2952& 0.83 \\
        
        \midrule
        KPAC + NeRF &26.40 &.8194 &.1624 &28.15 &.8592 &.0815 &26.69 &.6589 &.2631 &24.81 &.8147 &.1639 &23.42 &.7495 &.2155 &25.89 &.7803 &.1773&5.00\\
        Deblur-NeRF & 28.03 &.8628 &.1127 &31.85& .9175& .0481& 30.52 &.8246& .1901 &26.25 &.8517 &.0995 &25.18 &.8067 &.1436 &28.37 &.8527 &.1188& 20.0\\
        \midrule
        
        DeblurTensoRF & 27.01 & .8257 & .1393 & 30.39 & .8882 & .0910 & 27.41 & .6841 & .2542 & 24.36 & .7835 & .1276 & 23.91 & .7593 & .1564 & 26.62 & .7882 & .1537 & 1.50\\        
        
        $\textrm{PDRF}^{\textrm{single}}$-5 & 28.33 & .8743 & .1445 & 31.78 & .9222 & .0541 & 30.43 & \seccol{.8233} & .2318 & 26.26 & .8649 & .1194 & 25.47 & .8261 & .1652 & 28.45 & .8622 & .1430&\tp{1.15}\\        
        
        PDRF-5 & \seccol{30.34} & \seccol{.9032} & \seccol{.1378} & \seccol{32.10} & \seccol{.9269} & \seccol{.0503} & \seccol{30.48} & .8262 & \seccol{.2274} & \seccol{27.31} & .8818 & .1209 & 27.05 & .8581 &  .1501 & 29.46 & .8792 & .1373&1.33\\
        PDRF-10 & \tp{30.90} & \tp{.9138} & \tp{.1111} & \tp{32.29} & \tp{.9305} & \tp{.0437} & \tp{30.97} & \tp{.8408} & \tp{.1960} & \tp{28.18} & \tp{.9006} & \tp{.0877} & \tp{28.07} &  \tp{.8799} & \tp{.1196} & \tp{30.08} & \tp{.8931} & \tp{.1116}&2.33\\
        \bottomrule
        
        \end{tabular}\\
    \end{tabular}        
    \caption{}
    \label{tab:results}
    \vspace{-1em}
\end{table*}


==> figures/title.tex <==
\captionsetup{type=figure}
\noindent\begin{minipage}{\textwidth} 
\begin{minipage}{0.5\textwidth}
  \centering
    \begin{minipage}{0.32\textwidth}
      \centering
        % \vspace{-1.6em}
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/source/002.png}
                \caption{\fontsize{8}{10}\selectfont Source View 1}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/002_GT_marked.png}
                \caption{\fontsize{8}{10}\selectfont Novel View}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        % \vspace{-1.6em}
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/source/030.png}
                \caption{\fontsize{8}{10}\selectfont Source View 2}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/002_NeRF_crop.png}
                \caption{\fontsize{8}{10}\selectfont NeRF, 5 hrs}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/002_Plenoxel_crop.png}
                \caption{\fontsize{8}{10}\selectfont Plenoxel, 25 mins}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/002_TensoRF_crop.png}
                \caption{\fontsize{8}{10}\selectfont TensoRF, 50 mins}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/002_DeblurNeRF_crop.png}
                \caption{\fontsize{8}{10}\selectfont DeblurNeRF, \emph{20 hrs}}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/002_Ours_crop.png}
                \caption{\fontsize{8}{10}\selectfont Ours, \underline{\emph{80 mins}}}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/motion/002_GT_crop.png}
                \caption{\fontsize{8}{10}\selectfont Ground Truth}
        \end{subfigure}  
    \end{minipage}
\end{minipage}
\begin{minipage}{0.5\textwidth}
  \centering
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/028.png}
                \caption{\fontsize{8}{10}\selectfont Source View 1}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/032_GT_marked.png}
                \caption{\fontsize{8}{10}\selectfont Novel View}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/033.png}
                \caption{\fontsize{8}{10}\selectfont Source View 2}
        \end{subfigure}  
    \end{minipage}

    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/032_NeRF_crop.png}
                \caption{\fontsize{8}{10}\selectfont NeRF, }
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/032_Plenoxel_crop.png}
                \caption{\fontsize{8}{10}\selectfont Plenoxel, }
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/032_TensoRF_crop.png}
                \caption{\fontsize{8}{10}\selectfont TensoRF}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/032_DeblurNeRF_crop.png}
                \caption{\fontsize{8}{10}\selectfont DeblurNeRF}
        \end{subfigure}  
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/032_Ours_crop.png}
                \caption{\fontsize{8}{10}\selectfont Ours}
        \end{subfigure}  
    \end{minipage}    
    \begin{minipage}{0.32\textwidth}
      \centering
        \begin{subfigure}{\textwidth}
          \includegraphics[width=\linewidth]{figures/imgs/defocus/032_GT_crop.png}
                \caption{\fontsize{8}{10}\selectfont Ground Truth}
        \end{subfigure}  
    \end{minipage}
\end{minipage} 
\caption{figures} 
\label{fig:intro} 
\end{minipage}

==> figures/visualization.tex <==
%& $\textrm{XraySyn}_{ref}$ 
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[htb!]
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}[b]{ccccccc}
        % \hline
         NeRF & Plenoxel & TensoRF & Deblur-NeRF& PDRF & Ground Truth&Novel View\\

        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/002_NeRF_crop.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/002_Plenoxel_crop.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/002_TensoRF_crop.png}
            \caption{}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/002_DeblurNeRF_crop.png}
            \caption{}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/002_Ours_crop.png}
            \caption{}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/002_GT_crop.png}
            \caption{}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth]{figures/imgs/motion/002_GT_marked.png}
            \caption{}
        \end{subfigure} \\

        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus/024_nerf_crop.png}
            \caption{21.71/0.7980}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus/024_plenoxel_crop.png}
            \caption{20.80/0.7780}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus/024_tensorf_crop.png}
            \caption{19.33/0.7580}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus/024_deblur_crop.png}
            \caption{\seccol{23.91/0.8692}}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus/024_ours_crop.png}
            \caption{\tp{27.92/0.9281}}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus/024_gt_crop.png}
            \caption{PSNR/SSIM}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus/024_gt_marked.png}
            \caption{}
        \end{subfigure}\\ 



        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/motion_real/021_nerf_crop.png}
            \caption{18.06/0.5609}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/motion_real/021_plenoxel_crop.png}
            \caption{17.60/0.5970}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/motion_real/021_tensorf_crop.png}
            \caption{15.39/0.3749}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/motion_real/021_deblurnerf_crop.png}
            \caption{\seccol{21.52/0.7956}}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/motion_real/021_ours_crop.png}
            \caption{\tp{23.55/0.8361}}
        \end{subfigure} & 
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/motion_real/021_gt_crop.png}
            \caption{PSNR/SSIM}
        \end{subfigure} & 
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/motion_real/021_gt_marked.png}
            \caption{}
        \end{subfigure}\\ 


        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus_real_2/024_nerf_crop.png}
            \caption{23.06/0.6711}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus_real_2/024_plenoxel_crop.png}
            \caption{22.33/0.6269}
        \end{subfigure} &
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus_real_2/024_tensorf_crop.png}
            \caption{21.07/0.7647}
        \end{subfigure} &   
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus_real_2/024_deblur_crop.png}
            \caption{\tp{25.92}/\seccol{0.8513}}
        \end{subfigure} &  
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus_real_2/024_ours_crop.png}
            \caption{\seccol{24.82}/\tp{0.8800}}
        \end{subfigure} & 
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus_real_2/024_gt_crop.png}
            \caption{PSNR/SSIM}
        \end{subfigure} & 
        \begin{subfigure}[b]{0.14\linewidth}
            \includegraphics[width=\textwidth,height=\textwidth]{figures/imgs/defocus_real_2/024_gt_marked.png}
            \caption{}
        \end{subfigure}\\ 

        % \hline
    \end{tabular}
    \caption{Visual comparisons of different radiance field modeling methods. The first two rows are synthetic scenes with motion and defocus blur. The last two rows are real scenes with motion and defocus blur. For real scenes, the ground truth is for reference only as the exposure is often inconsistent with source views; PSNR and SSIM similarly only provide an estimate of quality. We color code \tp{best} and \seccol{second best} performances.}
    \label{tab:visualization}
    \vspace{-1.5em}
\end{figure*}
